Reversing Single Sessions

Session-based communication has gained a widespread acceptance in practice as a means for developing safe communicating systems via structured interactions. In this paper, we investigate how these structured interactions are affected by reversibility, which provides a computational model allowing executed interactions to be undone. In particular, we provide a systematic study of the integration of different notions of reversibility in both binary and multiparty single sessions. The considered forms of reversibility are: one for completely reversing a given session with one backward step, and another for also restoring any intermediate state of the session with either one backward step or multiple ones. We analyse the costs of reversing a session in all these different settings. Our results show that extending binary single sessions to multiparty ones does not affect the reversibility machinery and its costs.

==> tex/discussion.tex <==
% !TEX root = ../reversible_sessions@lics.tex
\section{Dicussion}
\label{sec:discussion}

We discuss in this section the key points of the results of our study and 
illustrate possible extensions of this research line involving other reversibility solutions.

The results summarised in Table~\ref{tab:costs} show that passing from binary sessions
to multiparty ones does not affect the reversibility machineries and their costs.
Instead, passing from single sessions to multiple ones has a significant impact. In terms of 
reversibility machinery, rather than using a single stack per session it is required a graph-like
data structure, in order to keep track of the causal dependences among the session 
interactions. This leads to an higher cost for enabling the reversibility (indeed, the natural numbers
$n$ and $m$ in Table~\ref{tab:costs} are such that $n \leq m$). This gap is due to the fact that
interactions along a single session are not affected by other sessions; this, in combination with 
linearity of session types, means that reverting interactions along a single session is like reverting 
a sequential computation. Instead, in the multiple sessions setting, the computation of a session 
can interleave with the computations of others. Thus, in this case reverting a session corresponds to
revert a concurrent computation in a causal-consistent way, which requires to revert interactions
performed along other sessions that have a casual dependence with the interactions of the session 
to be reverted. 


\bigskip
---------------------
\bigskip



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The calculi considered in this paper are \emph{fully} reversible, i.e. backward computations 
are always enabled. Thus, their semantics explains how sessions are reversed 
(i.e., which mechanisms are involved and which effects are produced) but does not
define when the rollback is triggered. 
%
Full reversibility provides theoretical foundations for studying reversibility in session-based 
\pic, but it is not suitable for a practical use on structured communication-based programming. 
In line with \cite{LaneseMSS11}, we plan to enrich the language with 
primitives and mechanisms to control reversibility.
%
Specifically, in a controlled approach for session reversibility, rollback could be 
activated by the synchronisation between the session parties via a specific $\mathbf{roll}$
primitive. For example, in the single binary session with whole session reversibility the 
backward rule \rulelabel{Bw(1)} would become
\begin{center}
\small
\begin{tabular}{l@{\quad }r}
$
\singleSes{s}{Q}\res{\tuple{c}}(P \mid \ce{k}:\mathbf{roll} \mid  k:\mathbf{roll} )
\ \bwred\ 
Q
$ 
& $(k=s\ \, \text{or}\ \, k=\ce{s})$
\end{tabular}
\end{center}
In this case, the two parties synchronise on their session endpoints to restore the 
process $Q$ stored in the memory stack.
 


==> tex/host_calculus.tex <==
% !TEX root = ../aplas2014.tex
\section{Background}
\label{sec:host_calculus}

\todo[inline]{The complete background can be left in the companion technical report, while it will be 
heavily shortened, or removed, in the submitted paper.  }

In this section, we present syntax, semantics and type discipline of the considered variants of \pic\ 
enriched with primitives for managing synchronous binary and multiparty sessions.
%\footnote{In particular, 
%we consider the well-established calculus introduced in \cite{YoshidaV07}, whose notation has been revised according to that used in 
%more recent works on binary session types (in particular, \cite{MostrousY09}).}.

\subsection{Binary session calculus}

%A (binary) session is a series of reciprocal interactions between two parties, possibly with branching and recursion. Interactions on a session are performed via a dedicated private channel, which is generated when initiating the session.

\subsubsection{Syntax.}
\label{sec:syntax_pic}
%We use the following base sets: 
%\emph{variables} (ranged over by $x$, $y$, \ldots),
%\emph{shared channels} (ranged over by $a$, $b$, \ldots),
%\emph{session channels} (ranged over by $s$, $s'$, \ldots), 
%\emph{session endpoints} (including session channels, ranged over by $s$, $s'$,\ldots, $\ce{s}$, $\ce{s\,}'$,\ldots),
%\emph{labels} (ranged over by $l$, $l'$, \ldots),
%and  \emph{process variables} (ranged over by $X$, $Y$, \ldots).
%%
%Letters $u$, $u'$, \ldots denote \emph{shared identifiers}, i.e. shared channels and variables together. 
%Letters $k$, $k'$, \ldots denote \emph{session identifiers}, i.e. session endpoints and variables together. 
%Letters $c$, $c'$, \ldots denote \emph{channels}, i.e. session channels and shared channels together. 
%%
%\emph{Values}, including boolean ($\ctrue$, $\cfalse$), integers (0, 1, \ldots) and shared channles
%and session endpoints, are ranged over by $v$, $v'$, \ldots.

We use the following base sets: 
\emph{shared channels}, used to initiate sessions;
\emph{session channels}, consisting on pairs of \emph{endpoints} used by the two parties 
to exchange \emph{values} within an established session;
\emph{variables}, used to store values;
\emph{labels}, used to select and offer branching choices;
and  \emph{process variables}, used for recursion. 
%
The corresponding notation and terminology are as follows:
$$
\hspace*{3cm}
\begin{array}{l}
\left.
\begin{array}{l}
\text{Variables:}\ x,y,\ldots\\[.1cm]
\text{Shared channels:}\ a,b,\ldots\\
\end{array}
\right\} \text{Shared identifiers:}\ u,u',\ldots
\vspace*{-.5cm}
\\
\hspace*{-3.04cm}
\text{Channels:}\ c,c',\ldots\left\{
\begin{array}{l}
\\[.09cm]
\text{Session channels}\ s,s'\ldots
\end{array}
\right.
\\[.3cm]
\left.
\begin{array}{l}
\text{Variables:}\ x,y,\ldots\\
\text{Session endpoints:}\ s,\ce{s},\ldots\\
\end{array}
\right\} \text{Session identifiers:}\ k,k',\ldots
\\[.4cm]
\hspace*{.1cm} \text{Labels:}\ l, l',\ldots\\
\hspace*{.1cm} \text{Process variables:}\ X, Y,\ldots\\
%
\end{array}
$$
%\\[-.2cm]
$$
\begin{array}{l}
%
\hspace*{-4.1cm}
\text{Values:}\ v,v',\ldots \left\{
\begin{array}{l}
\text{Booleans:}\ \ctrue,\cfalse\\
\text{Integers:}\ 0,1,\ldots\\
\text{Shared channels:}\ a,b,\ldots\\
\text{Session endpoints:}\ s,\ce{s},\ldots\\
\end{array}
\right.
\end{array}
$$
Notably, each session channel $s$ has two (dual) endpoints, denoted by $s$ and $\ce{s}$, 
each one assigned to one session party to exchange values with the other.  
We define duality to be idempotent, i.e. $\ce{\ce{s}}=s$.
The use of two separated endpoints is similar to that of \emph{polarities} in \cite{GayH05,YoshidaV07}. 

\emph{Processes}, ranged over by $P$, $Q$, \ldots, and 
\emph{expressions}, ranged over by $e$, $e'$, \ldots are given by the grammar in Figure~\ref{fig:syntax_pi}. 
We use $\text{op}(\cdot)$ to denote a generic expression operator; we assume that expressions 
are equipped with standard operators on boolean and integer values (e.g., $\wedge$, $+$, \ldots).
\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{rcl@{\hspace{-.1cm}}r}
	\textbf{Processes}\quad
	$P$ & ::= & $\requestAct{u}{x}{P}$ & connect\\
	& $\mid$ & $\acceptAct{u}{x}{P}$ & connect dual\\
	& $\mid$ & $\sendAct{k}{e}{P}$ & output\\
	& $\mid$ & $\receiveAct{k}{x}{P}$ & input\\
	& $\mid$ & $\selectAct{k}{l}{P}$ & selection\\
	& $\mid$ & $\branchAct{k}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$ & branching\\
	& $\mid$ & $\ifthenelseAct{e}{P}{Q}$ & conditional choice\\
	& $\mid$ & $P \mid Q$ & parallel composition\\
	& $\mid$ & $\res{c}\, P$ & restriction\\		
	& $\mid$ & $X$ & process variable\\
	& $\mid$ & $\recAct{X}{P}$ & recursion\\		
	& $\mid$ & $\inact$ & inaction\\	
	\\
	\textbf{Expressions}\quad
	%$e$ & ::= & $v \ \ \mid\ \ x \ \ \mid\ \ \text{op}(e_1,\ldots,e_n)$  & expressions
	$e$ & ::= & $v$ & value\\	
	& $\mid$ & $x$ & variable\\		
	& $\mid$ & $\text{op}(e_1,\ldots,e_n)$ & composed expression
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Binary session calculus: syntax}
	\label{fig:syntax_pi}
	\vspace*{-.4cm}
	\end{centering}
\end{figure}

The initiation of a session is triggered by the synchronisation on a shared channel $a$ 
of two processes of the form  $\requestAct{a}{x}{P}$ and 
$\acceptAct{a}{y}{Q}$.
This causes the generation of a fresh session channel $s$, 
whose endpoints replace variables $x$ and $y$, by means of a substitution application, 
in order to be used by $P$ and $Q$, respectively, for later communications. 
%
Primitives $\sendAct{k}{e}{P}$ and $\receiveAct{k'}{x}{Q}$ 
denote output and input via session endpoints identified by $k$ and $k'$, respectively. 
These communication primitives realise the standard synchronous message passing, where messages result 
from the evaluation of expressions. Notably, an exchanged value can be 
an endpoint that is being used in a session (this channel-passing modality is 
called \emph{delegation}), thus allowing complex nested structured communications. 
%
Constructs $\selectAct{k}{l}{P}$ and 
$\branchAct{k'}{\branch{l_1}{P_1}\branchSep\ldots\branchSep \branch{l_n}{P_n}}$
denote label selection and label branching (where $l_1$, \ldots, $l_n$ are assumed to 
be pairwise distinct) via endpoints identified by $k$ and $k'$, respectively. 
They mime method invocation in object-based programming. 
%

The above interaction primitives are then combined by standard process calculi 
constructs: 
conditional choice, parallel composition, restriction, 
recursion\footnote{The language presented so far slightly differs from \cite{YoshidaV07}, 
because we used recursion instead of process definitions. Indeed, recursion is easier to deal 
within a theoretical framework because the syntax of a recursive term already contains all the 
code needed to properly run the term itself.}
and the empty process (denoting inaction).
%
It is worth noticing that restriction can have both shared and session channels as argument:
$\res{a}P$ states that $a$ is a private shared channel of $P$; similarly, $\res{s}P$ states that 
the two endpoints of the session channel, namely $s$ and $\ce{s}$, are invisible from processes 
different from $P$ (see the seventh law in Figure~\ref{fig:congruence_pic}), 
i.e. no external process can perform a session action on either of these 
endpoints (this ensures non-interference within a session).
%
As a matter of notation, we will write %$\res{c_1,\ldots,c_n}P$
$\res{\tuple{c}}P$
in place of  $\res{c_1}\ldots\res{c_n}P$.

We adopt the following conventions about the operators precedence: 
prefixing, restriction, and recursion bind more tightly than parallel composition.

Bindings are defined as follows:
%
$\requestAct{u}{x}{P}$, $\acceptAct{u}{x}{P}$ and $\receiveAct{k}{x}{P}$
bind variable $x$ in $P$;
$\res{a}\, P$ binds shared channel $a$ in $P$;
%
$\res{s}\, P$ binds session channel $s$ in $P$;
%
finally, $\recAct{X}{P}$ binds process variable $X$ in $P$.
%
The derived notions of bound and free names, alpha-equivalence $\alphaeq$, and 
substitution are standard. 
For $P$ a process, 
$\freev{P}$ denotes the set of \emph{free variables}, 
$\freec{P}$ denotes the set of \emph{free shared channels},
and $\freese{P}$ the set of \emph{free session endpoints}. 
%We also define 
%$\freeu{P} = \freen{P} \cup \freec{P}$.
%
For the sake of simplicity, we assume that free and bound variables are always chosen 
to be different, and that bound variables are pairwise distinct; the same applies to names.
Of course, these conditions are not restrictive and can always be fulfilled by possibly 
using alpha-conversion.

\subsubsection{Semantics.}
The operational semantics is given in terms of a structural congruence and of a reduction relation. 
Notably, %\todo{Shall this be ensured by the type system?} 
the semantics is only defined for \emph{closed} terms, i.e. terms without free variables. 
Indeed, we consider the binding of a variable as its declaration (and initialisation), 
therefore free occurrences of variables at the outset in a term must be prevented 
since they are similar to uses of variables before their declaration in programs 
(which are considered as programming errors).

The \emph{structural congruence}, written $\congr$, is defined as the smallest congruence relation 
on processes that includes the equational laws shown in Figure~\ref{fig:congruence_pic}. 
These are the standard laws of \pic: 
the first three are the monoid laws for $\mid$ (i.e., it is associative and commutative, and has 
$\inact$ as identity element); 
the second four laws deal with restriction and enable 
garbage-collection of channels, scope extension and scope swap, respectively; 
the eighth law permits unfolding a recursion (notation $P\subst{Q}{X}$ denotes 
replacement of free occurrences of $X$ in $P$ by process $Q$);
the last law equates alpha-equivalent processes, i.e.~processes only differing in the identity of 
bound variables/channels.

%\begin{figure}[t]
%	\begin{centering}	
%	\begin{tabular}{l@{\qquad\ \ }l@{\qquad\ \ }l}	
%	$(P \mid Q) \mid R \congr P \mid (Q \mid R)$ 
%	&
%	$P \mid Q \congr Q \mid P$ 
%	&
%	$P \mid \inact \congr P$
%	\\[.3cm]
%	$\res{a}P \mid Q \congr \res{a}(P \mid Q)$\ \ if $a \notin \freec{Q}$
%	&
%	$\res{c_1}\res{c_2}P \congr \res{c_2}\res{c_1}P$
%	&
%	$\res{c} \inact \congr \inact$
%	\\[.3cm]
%	$\res{s}P \mid Q \congr \res{s}(P \mid Q)$\ \ if $s,\ce{s} \notin \freese{Q}$
%	&
%	$\recAct{X}{P} \congr P\subst{\recAct{X}{P}}{X}$
%	&
%	$P \congr Q$\ \ if $P \alphaeq Q$
%	\\[.2cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.2cm}
%	\caption{Session-based \pic: structural congruence}
%	\label{fig:congruence_pic}
%	%\vspace*{.4cm}
%	\end{centering}
%\end{figure}
\begin{figure}[t]
	\begin{centering}	
	\begin{tabular}{l@{\qquad\ \ }l}	
	$(P \mid Q) \mid R \congr P \mid (Q \mid R)$ 
	&
	$P \mid Q \congr Q \mid P$ 
	\\[.3cm]
	$P \mid \inact \congr P$
	&
	$\res{c} \inact \congr \inact$
	\\[.3cm]
	$\res{a}P \mid Q \congr \res{a}(P \mid Q)$\ \ if $a \notin \freec{Q}$
	&
	$\res{c_1}\res{c_2}P \congr \res{c_2}\res{c_1}P$
	\\[.3cm]
	$\res{s}P \mid Q \congr \res{s}(P \mid Q)$\ \ if $s,\ce{s} \notin \freese{Q}$
	&
	$\recAct{X}{P} \congr P\subst{\recAct{X}{P}}{X}$
	\\[.3cm]
	$P \congr Q$\ \ if $P \alphaeq Q$
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Binary session calculus: structural congruence}
	\label{fig:congruence_pic}
	\vspace*{-.4cm}
	\end{centering}
\end{figure}


To define the reduction relation, we use an auxiliary function $\expreval{\cdot}{\,}$ 
for evaluating closed expressions: 
$\expreval{e}{v}$ says that expression $e$ evaluates to value $v$ 
(where $\expreval{v}{v}$ and $\expreval{x}{\,}$ is undefined).

The \emph{reduction relation}, written $\red$, is the smallest relation on 
closed processes generated by the rules in Figure~\ref{fig:reduction_pic}.
%\begin{figure}[t]
%	\begin{centering}
%	\begin{tabular}{r@{\ \ }l@{\ \ }l@{\quad}l@{\quad}l}
%	$\requestAct{a}{x}{P_1}\ \mid \ \acceptAct{a}{y}{P_2}$
%	& $\red$ &
%	$\res{s}(P_1\subst{\ce{s}}{x} \mid P_2\subst{s}{y})$ 
%	& $s,\ce{s} \notin \freese{P_1,P_2}$ & \rulelabel{Con}
%	\\[.3cm]
%	$\sendAct{\ce{k}}{e}{P_1} \ \mid \ \receiveAct{k}{x}{P_2}$
%	& $\red$ &
%	$P_1 \mid P_2\subst{v}{x}$
%	& $(k=s\ \, \text{or}\ \, k=\ce{s}),\ \expreval{e}{v}$ & \rulelabel{Com}
%	\\[.3cm]
%	$\selectAct{\ce{k}}{l_i}{P} \ \mid \ \branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}$
%	& $\red$ &
%	$P \mid P_i$
%	& $(k=s\ \, \text{or}\ \, k=\ce{s}),\ 1 \leq i \leq n$ & \rulelabel{Lab}
%	\\[.3cm]
%	$\ifthenelseAct{e}{P_1}{P_2}$
%	& $\red$ &
%	$P_1$
%	& $\expreval{e}{\ctrue}$ & \rulelabel{If1}
%	\\[.3cm]
%	$\ifthenelseAct{e}{P_1}{P_2}$
%	& $\red$ &
%	$P_2$
%	& $\expreval{e}{\cfalse}$ & \rulelabel{If2}
%	\\[.3cm]
%%	$P \ \red\ P' \quad \imply\quad P \mid \ Q$
%%	& $\red$ &
%%	$P' \mid Q$
%%	& & \rulelabel{Par}
%%	\\[.3cm]
%%	$P \ \red\ P' \quad \imply\quad \res{c}P$
%%	& $\red$ &
%%	$\res{c}P'$
%%	& & \rulelabel{Res}
%%	\\[.3cm]
%%	$P \congr P'\ $ and $\ P' \, \red\, Q'\ $ and $\ Q \congr Q' \quad \imply \quad P$
%%	& $\red$ &
%%	$Q$
%%	& & \rulelabel{Str}
%	\end{tabular}
%	\begin{tabular}{c}
%	$
%	\infer[$\ \rulelabel{Par}$]{P \mid \ Q \ \red\ P' \mid Q}
%	{P \ \red\ P'}
%	$	
%	\qquad\qquad
%	$
%	\infer[$\ \rulelabel{Res}$]{\res{c}P \ \red\ \res{c}P'}
%	{P \ \red\ P'}
%	$
%	\qquad\qquad
%	$
%	\infer[$\ \rulelabel{Str}$]{P \ \red\ Q}
%	{P \congr P'\ \red\ Q' \congr Q}
%	$
%	\\[.2cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.2cm}
%	\caption{Session-based \pic: reduction relation}
%	\label{fig:reduction_pic}
%	%\vspace*{-.4cm}
%	\end{centering}
%\end{figure}
\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{l@{\quad}l@{\quad}l}
	$\requestAct{a}{x}{P_1}\ \mid \ \acceptAct{a}{y}{P_2}$
	$\ \red\ $
	$\res{s}(P_1\subst{\ce{s}}{x} \mid P_2\subst{s}{y})$ 
	& $s,\ce{s} \notin \freese{P_1,P_2}$ & \rulelabel{Con}
	\\[.3cm]
	$\sendAct{\ce{k}}{e}{P_1} \ \mid \ \receiveAct{k}{x}{P_2}$
	$\ \red\ $
	$P_1 \mid P_2\subst{v}{x}$
	& $(k=s\ \, \text{or}\ \, k=\ce{s}),\ \expreval{e}{v}$ & \rulelabel{Com}
	\\[.3cm]
	$\selectAct{\ce{k}}{l_i}{P} \ \mid \ \branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}$
	$\ \red\ $
	$P \mid P_i$
	& $(k=s\ \, \text{or}\ \, k=\ce{s}),\ 1 \leq i \leq n$ & \rulelabel{Lab}
	\\[.3cm]
	$\ifthenelseAct{e}{P_1}{P_2}$
	$\ \red\ $
	$P_1$
	& $\expreval{e}{\ctrue}$ & \rulelabel{If1}
	\\[.3cm]
	$\ifthenelseAct{e}{P_1}{P_2}$
	$\ \red\ $
	$P_2$
	& $\expreval{e}{\cfalse}$ & \rulelabel{If2}
	\\[.3cm]
	\end{tabular}
	\begin{tabular}{c}
	$
	\infer[$\,\rulelabel{Par}$]{P \mid \ Q \ \red\ P' \mid Q}
	{P \ \red\ P'}
	$	
	\qquad
	$
	\infer[$\,\rulelabel{Res}$]{\res{c}P \ \red\ \res{c}P'}
	{P \ \red\ P'}
	$
	\qquad
	$
	\infer[$\,\rulelabel{Str}$]{P \ \red\ Q}
	{P \congr P'\ \red\ Q' \congr Q}
	$
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}
	\caption{Binary session calculus: reduction relation}
	\label{fig:reduction_pic}
	\vspace*{.6cm}
	\end{centering}
\end{figure}
We comment on salient points. 
%
A new session is established when two parallel processes synchronise 
via a shared channel $a$; this results on the generation of a fresh (private) session 
channel whose endpoints are assigned to the two session parties (rule \rulelabel{Con}).
%
Along a session, the two parties can exchange values (for data- and channel-passing, 
rule \rulelabel{Com}) and labels (for branching selection, rule \rulelabel{Lab}). 
%
The other rules are standard and state that: 
conditional choice evolves according to the evaluation of the expression argument 
(rules \rulelabel{If1} and \rulelabel{If2});
if a part of a larger process evolves, the whole process evolves accordingly 
(rules \rulelabel{Par} and \rulelabel{Res});
and structural congruent processes have the same reductions (rule \rulelabel{Str}). 


%\subsection{Multiple providers scenario: session-based \pic}
%\label{sec:example}
%
%%We introduce here a simple scenario that will be used throughout the paper as a running 
%%example to illustrate our approach. 
%%The considered scenario involves a \emph{client} and multiple \emph{providers} offering 
%%the same service (e.g., on-demand video streaming). 
%%The client starts by opening a session with a provider (corresponding to the login phase)
%%and sends its service request (e.g., title of a movie, video quality, minimum bandwidth, etc.). 
%%Then, the provider sends a quote for the request determined according to the requested 
%%quality of service and to the servers status (e.g., current load, available bandwidth, etc.). 
%%The client can either accept, negotiate or reject the quote. In the first two cases,
%%the interaction between the two parties shall continue. 
%
%The scenario involving a client and multiple providers introduced in Section~\ref{sec:intro} 
%can be rendered in \mbox{\pic}\ as follows (for the sake of simplicity,
%here we consider just two providers):
%$$
%P_{client}  \ \mid \ P_{provider1}  \ \mid \ P_{provider2}  
%$$
%where the client process $P_{client}$ is defined as
%$$
%\begin{array}{l}
%\requestPrefix{a_{login}}{x}.\,\send{x}{\mathsf{srv\_req}}.\,\receive{x}{y_{quote}}.\\
%\quad
%\ifPi\ accept(y_{quote})\ \thenPi\ \selectAct{x}{l_{acc}}{\,P_{acc}}\\
%%\hspace*{4.5cm}
%\quad
%\elsePi\ (\ifPi\ negotiate(y_{quote})\ \thenPi\ \selectAct{x}{l_{neg}}{\,P_{neg}}\ 
%\elsePi\ \selectAct{x}{l_{rej}}{\,\inact})
%\end{array}
%$$
%while a provider process $P_{provider\,i}$ is as follows
%$$
%\begin{array}{l}
%\acceptPrefix{a_{login}}{y}.\,\receive{y}{z_{req}}.\,\send{y}{quote_i(z_{req})}.\,
%\branchAct{y}{\branch{l_{acc}}{Q_{acc}} \ \branchSep\ \branch{l_{neg}}{Q_{neg}} \ \branchSep\ \branch{l_{rej}}{\inact}}
%\end{array}
%$$
%
%We show below a possible evolution of the system, where the client contacts $provider1$ and 
%accepts the proposed quote: 
%$$
%\begin{array}{l}
%P_{client}  \ \mid \ P_{provider1}  \ \mid \ P_{provider2}  
%\\[.1cm]
%\red
%\\[.1cm]
%\res{s}(\,\send{\ce{s}}{\mathsf{srv\_req}}.\,\receive{\ce{s}}{y_{quote}}.\,
%\ifPi\ accept(y_{quote})\ \thenPi\ \selectAct{\ce{s}}{l_{acc}}{\,P_{acc}\subst{\ce{s}}{x}}
%\elsePi\ (\ldots)
%\\
%\hspace{.8cm}
%\mid\ 
%\receive{s}{z_{req}}.\,\send{s}{quote_i(z_{req})}.\,
%\branchAct{s}{\branch{l_{acc}}{Q_{acc}\subst{s}{y}} \ \branchSep\ \branch{l_{neg}}{Q_{neg}\subst{s}{y}} \ \branchSep\ \branch{l_{rej}}{\inact}}\,)
%\\
%\mid \ P_{provider2}  
%\\[.1cm]
%\red
%\\[.1cm]
%\res{s}(\,\receive{\ce{s}}{y_{quote}}.\,
%\ifPi\ accept(y_{quote})\ \thenPi\ \selectAct{\ce{s}}{l_{acc}}{\,P_{acc}\subst{\ce{s}}{x}}
%\elsePi\ (\ldots)
%\\
%\hspace{.8cm}
%\mid\ 
%\send{s}{quote_i(\mathsf{srv\_req})}.\,
%\branchAct{s}{\branch{l_{acc}}{Q_{acc}\subst{s}{y}\subst{\mathsf{srv\_req}}{z_{req}}} \ \branchSep\  \ldots}\,)
%\\
%\mid \ P_{provider2}  
%\\[.1cm]
%\red
%\\[.1cm]
%\res{s}(\,\ifPi\ accept(\mathsf{quote})\ \thenPi\ \selectAct{\ce{s}}{l_{acc}}{\,P_{acc}\subst{\ce{s}}{x}\subst{\mathsf{quote}}{y_{quote}}}
%\elsePi\ (\ldots)
%\\
%\hspace{.8cm}
%\mid\ 
%\branchAct{s}{\branch{l_{acc}}{Q_{acc}\subst{s}{y}\subst{\mathsf{srv\_req}}{z_{req}}} \ \branchSep\  \ldots}\,)
%\\
%\mid \ P_{provider2}  
%\\[.1cm]
%\red
%\\[.1cm]
%%\\[.1cm]
%%\red
%%\end{array}
%%$$
%%$$
%%\begin{array}{l}
%%\red
%%\\[.1cm]
%\res{s}(\,\selectAct{\ce{s}}{l_{acc}}{\,P_{acc}\subst{\ce{s}}{x}\subst{\mathsf{quote}}{y_{quote}}}
%\\
%\hspace{.8cm}
%\mid\ 
%\branchAct{s}{\branch{l_{acc}}{Q_{acc}\subst{s}{y}\subst{\mathsf{srv\_req}}{z_{req}}} \ \branchSep\  \ldots}\,)
%\\
%\mid \ P_{provider2}  
%\\[.1cm]
%\red
%\\[.1cm]
%\res{s}(\,P_{acc}\subst{\ce{s}}{x}\subst{\mathsf{quote}}{y_{quote}} \ \mid \
%Q_{acc}\subst{s}{y}\subst{\mathsf{srv\_req}}{z_{req}} \,)
%\\
%\mid \ P_{provider2}  
%
%\end{array}
%$$
%
%
%



\subsubsection{Type discipline.}
\label{sec:typingPic}

The type discipline presented here is a minor revision of the one proposed in 
\cite{YoshidaV07}, that takes into account the changes applied to the considered 
version of the binary session calculus (discussed in Section~\ref{sec:syntax_pic}).

\paragraph{Types.}
The syntax of \emph{sorts}, ranged over by $S$, $S'$, \ldots, and \emph{types}, ranged over by $\alpha$, 
$\beta$, \ldots, is defined in Figure~\ref{fig:typeSyntax}.
%
\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{rcl@{\hspace{-.1cm}}r}
	\textbf{Sorts}\quad
	$S$ & ::= & $\boolType$ & boolean\\
	& $\mid$ & $\intType$ & integer\\
	& $\mid$ & $\sharedChanType{\alpha}$ & shared channel\\
	\\
	\textbf{Types}\quad
	$\alpha$ & ::= & $\outType{S}.\alpha$ & output\\	
	& $\mid$ & $\inpType{S}.\alpha$ & input\\		
	& $\mid$ & $\thrType{\beta}.\alpha$ & throw\\		
	& $\mid$ & $\catType{\beta}.\alpha$ & catch\\			
	& $\mid$ & $\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ & selection\\			
	& $\mid$ & $\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ & branching\\				
	& $\mid$ & $\inactType$ & end\\
	& $\mid$ & $t$ & type variable\\
	& $\mid$ & $\recType{t}.\alpha$ & recursion
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Syntax of sorts and types}
	\label{fig:typeSyntax}
	\vspace*{-.4cm}
	\end{centering}
\end{figure}
%
The type $\outType{S}.\alpha$ represents the behaviour of first outputting a value of sorts $S$, 
then performing the actions prescribed by type $\alpha$; 
type $\thrType{\beta}.\alpha$ represents a similar behaviour, which starts with session output 
(\emph{throw}) instead; 
types $\inpType{S}.\alpha$ and $\catType{\beta}.\alpha$ are the dual ones, 
receiving values instead of sending. 
%
Type $\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ describes a branching 
behaviour: it waits with $n$ options, and behave as type $\alpha_i$ if the $i$-th action is selected 
(external choice); 
type $\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ then represents the behaviour 
which would select one of $l_i$ and then behaves as $\alpha_i$, according to the selected $l_i$ 
(internal choice). Type $\inactType$ represents inaction, acting as the unit of sequential composition.
%
Type $\recType{t}.\alpha$ denotes a recursive behaviour, representing the behaviour that starts 
by doing $\alpha$ and, when variable $t$ is encountered, recurs to $\alpha$ again. 
%
As in \cite{YoshidaV07}, we take an \emph{equi-recursive} view of types, not distinguishing between 
a type $\recType{t}.\alpha$ and its unfolding $\alpha\subst{\recType{t}.\alpha}{t}$, and we are 
interested on \emph{contractive} types only, i.e. for each of sub-expressions 
$\recType{t}.\recType{t_1}\ldots\recType{t_n}.\alpha$  the body $\alpha$ is not $t$. 
%
Thus, in a typing derivation, types $\recType{t}.\alpha$ and $\alpha\subst{\recType{t}.\alpha}{t}$ can be used interchangeably. 

For each type $\alpha$, we define $\dual{\alpha}$, the \emph{dual type} of $\alpha$, 
by exchanging $!$ and $?$, and $\&$ and $\oplus$. The inductive definition is in Figure~\ref{fig:dualType}.
%
\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{@{\hspace*{-.3cm}}r@{\ }c@{\ }l@{\qquad}r@{\ }c@{\ }l@{\qquad}r@{\ }c@{\ }l@{\qquad}r@{\ }c@{\ }l}
	$\dual{\outType{S}.\alpha}$ & = & $\inpType{S}.\dual{\alpha}$
	&
	$\dual{\outType{\beta}.\alpha}$ & = & $\inpType{\beta}.\dual{\alpha}$	
	&
	$\dual{\selType{\branch{l_i}{\alpha_i}}_{i\in I}}$ & = & $\branchType{\branch{l_i}{\dual{\alpha_i}}}_{i\in I}$
	&
	$\dual{\inactType}$ & = & $\inactType$
	\\[.3cm]
	$\dual{\inpType{S}.\alpha}$ & = & $\outType{S}.\dual{\alpha}$	
	&
	$\dual{\inpType{\beta}.\alpha}$ & = & $\outType{\beta}.\dual{\alpha}$	
	&
	$\dual{\branchType{\branch{l_i}{\alpha_i}}_{i\in I}}$ & = & $\selType{\branch{l_i}{\dual{\alpha_i}}}_{i\in I}$	
	&
	\multicolumn{3}{l}{$\dual{\recType{t}.\alpha} \,=\, \recType{t}.\dual{\alpha}
	\quad \dual{t}\,=\,t$}
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Dual types}
	\label{fig:dualType}
	\vspace*{-.4cm}
	\end{centering}
\end{figure}
%

\paragraph{Typing System.}
A \emph{sorting} (resp. a \emph{typing}, resp. a \emph{basis}) is a finite partial map from 
shared identifiers to sorts (resp. from session identifiers to types, resp. from process variables to typings). 
We let $\sorting$, $\sorting'$, \ldots (resp. $\typing$, $\typing'$, \ldots, 
resp. $\basis$, $\basis'$, \ldots) range over sortings (resp. typings, resp. bases).
%
We write $\typing \comp k:\alpha$ when $k \notin dom(\typing)$;
this notation is then extended to $\typing \comp \typing'$. 

Typing judgement are of the form $\basis;\sorting \judge P \hasType \typing$
which stands for ``under the environment $\basis;\sorting$, process $P$ has typing $\typing$''. 
The typing system is defined by the axioms and rules in Figure~\ref{fig:typingSysytem}. 
We call a typing \emph{completed} when it contains only $\inactType$ types. 
A typing $\typing$ is called \emph{balanced} if  whenever $s:\alpha,\ce{s}:\beta\in \typing$, then $\alpha=\dual{\beta}$.
%
We refer the interested reader to \cite{YoshidaV07} for detailed comments on the rules
and results.

\begin{figure}[!t]
	\begin{centering}
	\begin{tabular}{@{\hspace*{-2cm}}c}
	$\sorting \judge \ctrue \hasType \boolType$\ \ \rulelabel{Bool$_{\mathit{tt}}$}
	\qquad
	$\sorting \judge \cfalse \hasType \boolType$\ \ \rulelabel{Bool$_{\mathit{ff}}$}
	\qquad
	$\sorting \judge 1 \hasType \intType$\ \ \rulelabel{Int}	
	\qquad \ldots
	\\[.4cm]
	$
	\infer[$\ \rulelabel{Sum}$]{\sorting \judge +(e_1,e_2) \hasType \intType}
	{\sorting \judge e_1 \hasType \intType & & \sorting \judge e_2 \hasType \intType}
	$		
	\qquad
	$
	\infer[$\ \rulelabel{And}$]{\sorting \judge \wedge(e_1,e_2) \hasType \boolType}
	{\sorting \judge e_1 \hasType \boolType & & \sorting \judge e_2 \hasType \boolType}
	$		
	\qquad \ldots
	\\[.2cm]
	\end{tabular}
	\begin{tabular}{@{\hspace*{-2cm}}r@{\hspace*{.4cm}}r}
	$\sorting\comp u:S \judge u \hasType S$\ \ \rulelabel{Id}	
	&
	\infer[$\ \rulelabel{Inact}$]{\basis;\sorting \judge \inact \hasType \typing}
	{\typing\ \  \text{completed}}	
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Req}$]{\basis;\sorting \judge \requestAct{u}{x}{P} \hasType \typing}
	{\sorting \judge u \hasType \sharedChanType{\alpha} & & \basis;\sorting \judge P \hasType \typing\comp x:\dual{\alpha}}
	$		
	&
	$
	\infer[$\ \rulelabel{Acc}$]{\basis;\sorting \judge \acceptAct{u}{x}{P} \hasType \typing}
	{\sorting \judge u \hasType \sharedChanType{\alpha} & & \basis;\sorting \judge P \hasType \typing\comp x:\alpha}
	$		
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Send}$]{\basis;\sorting \judge \sendAct{k}{e}{P} \hasType \typing\comp k:\outType{S}.\alpha}
	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType \typing\comp k:\alpha}
	$		
	&
	$
	\infer[$\ \rulelabel{Thr}$]{\basis;\sorting \judge \sendAct{k}{k'}{P} \hasType \typing\comp k:\thrType{\alpha}.\beta\comp k':\alpha}
	{\basis;\sorting \judge P \hasType \typing\comp k:\beta}
	$		
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Rcv}$]{\basis;\sorting \judge \receiveAct{k}{x}{P} \hasType \typing\comp k:\inpType{S}.\alpha}
	{\basis;\sorting\comp x:S \judge P \hasType \typing\comp k:\alpha}
	$		
	&
	$
	\infer[$\ \rulelabel{cat}$]{\basis;\sorting \judge \receiveAct{k}{x}{P} \hasType \typing\comp k:\catType{\alpha}.\beta}
	{\basis;\sorting \judge P \hasType \typing\comp k:\beta \comp x:\alpha}
	$		
	\\[.4cm]	
	\multicolumn{2}{c}{	
	$
	\infer[(1 \leq j \leq n)\  $\ \rulelabel{Sel}$]{\basis;\sorting \judge \selectAct{k}{l_j}{P} \hasType \typing
	\comp k:\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}}
	{\basis;\sorting  \judge P \hasType \typing \comp k:\alpha_j}
	$}
	\\[.4cm]	
	\multicolumn{2}{c}{	
	$
	\infer[$\ \rulelabel{Br}$]{\basis;\sorting \judge \branchAct{k}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}} \hasType \typing
	\comp k:\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}}
	{\basis;\sorting  \judge P_1 \hasType \typing \comp k:\alpha_1 && \ldots 
	 && \basis;\sorting  \judge P_n \hasType \typing \comp k:\alpha_n}
	$}
	\\[.4cm]		
	\multicolumn{2}{c}{
	$
	\infer[$\ \rulelabel{If}$]{\basis;\sorting \judge \ifthenelseAct{e}{P}{Q} \hasType \typing}
	{\sorting  \judge e \hasType \boolType &&
	\basis;\sorting  \judge P \hasType \typing && \basis;\sorting  \judge Q \hasType \typing}
	$}	
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Conc}$]{\basis;\sorting \judge P\mid Q \hasType \typing\comp \typing'}
	{\basis;\sorting  \judge P \hasType \typing && \basis;\sorting  \judge Q \hasType \typing'}
	$		
	&
	$
	\infer[$\ \rulelabel{Res1}$]{\basis;\sorting \judge \res{a}{P} \hasType \typing}
	{\basis;\sorting\comp a:S  \judge P \hasType \typing}
	$	
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Res2}$]{\basis;\sorting \judge \res{s}{P} \hasType \typing}
	{\basis;\sorting  \judge P \hasType \typing\comp s:\alpha \comp \ce{s}:\dual{\alpha}}
	$	
	&
	$
	\infer[$\ \rulelabel{Res3}$]{\basis;\sorting \judge \res{s}{P} \hasType \typing}
	{\basis;\sorting  \judge P \hasType \typing && s\ \text{ not in }\ \typing}
	$	
	\\[.4cm]	
	$\basis\comp X:\typing;\sorting \judge X \hasType \typing$\ \ \rulelabel{Var}			
	&
	\infer[$\ \rulelabel{Rec}$]{\basis;\sorting \judge \recAct{X}{P} \hasType \typing}
	{\basis\comp X:\typing;\sorting  \judge P \hasType \typing}	
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}
	\caption{Typing System for binary session calculus}
	\label{fig:typingSysytem}
	\vspace*{-.4cm}
	\end{centering}
\end{figure}


==> tex/irreversibleSessions.tex <==
% !TEX root = ../reversible_sessions_TR.tex
\section{Commitable sessions}
\label{sec:irrev_calculus}

The calculus \respi\ discussed so far is \emph{fully} reversible, i.e. backward computations are always enabled. 
Full reversibility provides theoretical foundations for studying reversibility in session-based \pic, 
but it is not suitable for a practical use on structured communication-based programming. 
%
Therefore, in this section, we enrich the framework to allow computation go backward and
forward along a session, allowing the involved parties to try different interactions, until the session 
is successfully completed. This is achieved by adding a specific action to the calculus for irreversibly committing 
the closure of a sessions. 

It is worth noticing that the fully reversible characterisation of the calculus permits proving 
that its machineries for reversibility (i.e., memories and their usage) soundly works  with 
respect to the expected properties of a reversible calculus, and this  remains valid also for 
the extension proposed here. In fact, as clarified below, basically the extended calculus just
prunes some computations allowed in \respi, which corresponds to forward and backward 
actions that are undesired after a session closure.

\subsection{\respi\ with \texttt{commit}}
The syntax of \respic\ (\emph{Reversible Session-based} $\pi$ \emph{with Commit}) 
is obtained from that of \respi (given in Figure~\ref{fig:syntax_respi}) by extending
the syntactic category of processes $P$ with process $\commitAct{k}{P}$ 
and by extending the syntactic category of memories $m$ with the \emph{commit memory}
$\commem{t_1}{s}{t_2}$. This new memory simply registers the closing event of the session
identified by $s$ due to an agreement of threads tagged $t_1$ and $t_2$.

The irreversible closure of a session is achieved by the synchronisation on its session channel $s$ 
of two threads of the form  \mbox{$\ptag{t_1}\commitAct{\ce{s}}{P_1}$} and 
$\ptag{t_2}\commitAct{s}{P_2}$. After this synchronisation, since the session $s$ is closed,
the continuations $P_1$ and $P_2$ should not use any more the session channel $s$; this 
check is statically enforced by the type system for \respic\ (presented later on).  

Formally, the semantics of \respic\ is obtained by adding the following rule to those 
defining the reduction relation of \respi\ (Figure~\ref{fig:reduction_respi}): 
\begin{center}
\begin{tabular}{@{}l@{\hspace*{.3cm}}r@{\quad}l@{}}
	$\ptag{t_1}\commitAct{\ce{k}}{P_1} \ \mid \ \ptag{t_2}\commitAct{k}{P_2}$
	& $(k=s\ \, \text{or}\ \, k=\ce{s})$ &\rulelabel{commit}
	\\[.1cm]
	\quad $\fwred\ \  \res{t_1',t_2'}(
	\ptag{t_1'}P_1 \mid \ptag{t_2'}P_2
	\mid \commem{t_1}{s}{t_2})$	
\end{tabular}
\end{center}
Since $\texttt{commit}$ is an irreversible action that will never be backtracked, there is 
no need to remember information about the continuation processes in the generated 
memory. For the same reason, there is no backward rule inverse to \rulelabel{commit}. 

For what concerns the type discipline, types $\alpha$ (defined in Table~\ref{fig:typeSyntax}) 
are extended with type $\commitType$, while the typing system is extended with the following rule:  
$$
	\infer[$\ \rulelabel{Commit}$]{\basis;\sorting \judge \commitAct{k}{P} \hasType \typing\comp k:\commitType}
	{\basis;\sorting \judge P \hasType \typing\comp k:\inactType}
$$		
which ensures that after the commit the session is closed. 


\subsection{Irreversibility propagation}
When a $\texttt{commit}$ action is executed, all actions that caused it became unbacktrackable, 
although they were themselves reversible. In other words, a $\texttt{commit}$ action
create a \emph{domino effect} that disables the possibility of reverse the session actions
previously performed.

To formalise the domino effect caused by the $\texttt{commit}$ irreversible action, we
have to introduce the following notions of \emph{head} and \emph{tail} of memories:
$$
\begin{array}{l@{\qquad\quad}l}
\mhead{\amem{\actEv{t_1}{\storedAct}{t_2}}{t_1'}{t_2'}} \, = \, \{t_1,t_2\}
&
\mtail{\amem{\actEv{t_1}{\storedAct}{t_2}}{t_1'}{t_2'}} \, = \, \{t_1',t_2'\}
\\[.2cm]
\mhead{\cmem{t}{\ifEv{e}{P}{Q}}{t'}} \, = \, \{t\}
&
\mtail{\cmem{t}{\ifEv{e}{P}{Q}}{t'}} \, = \, \{t'\}
\\[.2cm]
\mhead{\fmem{\fev{t}{t_1}{t_2}}} \, = \, \{t\}
&
\mtail{\fmem{\fev{t}{t_1}{t_2}}} \, = \, \{t_1,t_2\}
\\[.2cm]
\mhead{\commem{t_1}{s}{t_2}} \, = \, \{t_1,t_2\}
&
\mtail{\commem{t_1}{s}{t_2}} \, = \, \emptyset
\end{array}
$$  

Using the terminology of \cite{DanosK04}, we say that a memory is \emph{locked}
when the event stored inside can never be reverted, because the conditions
triggering the corresponding backward reduction will never be satisfied. 
Specifically, to perform a backward reduction is required the coexistence 
of a memory with threads properly tagged, and the latter will never be available 
due to an irreversible action. Let us now formalise, given a process $M$, 
its set $\lockedmemset{M}$ of locked memories.

\begin{definition}[Locked memories]\label{def:locked}
Let $M$ be a \respic\ process and $\memset{M}$ stand for the set of memories 
occurring in $M$. 
%
The set $\lockedmemset{M}$ of locked memories of $M$ is defined as follows:
\begin{itemize}
\item $\commem{t_1}{s}{t_2} \in \memset{M} 
\quad \Rightarrow \quad 
\commem{t_1}{s}{t_2} \in \lockedmemset{M}$
\\[-.25cm]
\item $m \in \lockedmemset{M}$, $m' \in \memset{M}$, $t\in \mhead{m}$, $t\in \mtail{m'}
\quad \Rightarrow \quad 
m' \in \lockedmemset{M}$
\end{itemize}
\end{definition}
The first point says that a commit memory is locked, while the second point describes
the propagation of the locking effect, i.e. the event within $m$ depends on the event within $m'$
(because the latter generates a thread involved in the former) and hence also $m'$ is locked.
Of course, $\lockedmemset{M} \subseteq \memset{M}$.

It is worth noticing that \texttt{commit} must be carefully used in case of 
subordinate sessions. For example, in the typical three-party scenario
where a \emph{Customer} sends an order to a \emph{Seller} that, in his own turn, 
contacts a \emph{Shipper} for the delivery, we have that the session between the
\emph{Shipper} and the \emph{Seller} is subordinated to the session between
the \emph{Customer} and the \emph{Seller}. Now, when the main session is 
committed, also the subordinate session is involved in the commit, This is usually
desirable, because the commit acts on the whole transaction and, hence, after 
the commit the interaction with the \emph{Shipper} cannot be reverted. 
However, if the subordinate session is previously committed, the main session 
is affected because interaction performed before the commit cannot be reverted. 
This latter situation is typically undesired; therefore, as a best practice, \texttt{commit}
should be not used by subordinate sessions.  
  
 \subsection{Multiple providers scenario: \respic}\label{sec:examplerespic}
Let us consider again the multiple providers scenario 
specified in \respi\ in Section~\ref{sec:examplerespi}. 

Suppose now that, for the sake of simplicity, the client and the first provider 
commit the session immediately after the acceptance of the quote, i.e.
$P_{acc}$ and $Q_{acc}$ stand for $\commit{x}$ and $\commit{y}$,
respectively.
%
Thus, the computation described in Section~\ref{sec:example} in \respic\ corresponds to:
$$
\begin{array}{l@{\ }l}
\multicolumn{2}{l}{
\ptag{t_1}P_{client}  \ \mid \ \ptag{t_2}P_{provider1}  \ \mid \ \ptag{t_3}P_{provider2}  
}
\\[.1cm]
\multicolumn{2}{l}{
\fwred\ \fwred\ \fwred\ \fwred\ \fwred
}
\\[.1cm]
M \ = & \res{s,t_1^1,t_2^1,\ldots,t_1^4,t_2^4}
\\
&
(\,\ptag{t_1^4}\commit{\ce{s}} \ \mid \
\ptag{t_2^4}\commit{s} 
\\
&
\ \ \mid \
\amem{\actEv{t_1}{a_{login}\ldots}{t_2}}{t_1^1}{t_2^1}
\ \mid \ \ldots \ \mid \ 
\amem{\actEv{t_1^4}{\select{s}{l_{acc}}\ldots}{t_2^3}}{t_1^4}{t_2^4}
\,)
\\
&
\mid \ P_{provider2}  
\end{array}
$$
Now, $M$ can evolve as follows:
$$
\begin{array}{l@{\ }l}
M \fwred\ M' \ = & \res{s,t_1^1,t_2^1,\ldots,t_1^4,t_2^4,t_1^5,t_2^5}
\\
&
(\,\ptag{t_1^5}\inact \ \mid \
\ptag{t_2^5}\inact
\ \mid\ \commem{t_1^4}{s}{t_2^4}
\\
&
\ \ \mid \
\amem{\actEv{t_1}{a_{login}\ldots}{t_2}}{t_1^1}{t_2^1}
\ \mid \ \ldots \ \mid \ 
\amem{\actEv{t_1^4}{\select{s}{l_{acc}}\ldots}{t_2^3}}{t_1^4}{t_2^4}
\,)
\\
&
\mid \ P_{provider2}  
\end{array}
$$
The memory $\commem{t_1^4}{s}{t_2^4}$ generated by this last forward reduction
is locked (first point of Definition~\ref{def:locked}). 
Thus, also memory $\amem{\actEv{t_1^4}{\select{s}{l_{acc}}\ldots}{t_2^3}}{t_1^4}{t_2^4}$
is locked, since its tail contains tags belonging to the head of the commit memory  
(second point of Definition~\ref{def:locked}). Repeatedly  applying the second point of 
Definition~\ref{def:locked}, we obtain that $\lockedmemset{M'} = \memset{M'}$, i.e.
all memory of $M'$ are blocked. This means that $M'\not\bwred$ and hence, as desired, the 
computation along session $s$ cannot be reverted.





==> tex/multipleSession.tex <==
% !TEX root = ../reversible_sessions@fossacs.tex
\section{On reversing multiple sessions: a glimpse}
\label{sec:rev_multiple_sessions}

\todo[inline]{TODO}

\ifall


The results summarised in Table~\ref{tab:costs} show that passing from binary sessions
to multiparty ones does not affect the reversibility machineries and their costs.
Instead, passing from single sessions to multiple ones has a significant impact. In terms of 
reversibility machinery, rather than using a single stack per session it is required a graph-like
data structure, in order to keep track of the causal dependences among the session 
interactions. This leads to an higher cost for enabling the reversibility (indeed, the natural numbers
$n$ and $m$ in Table~\ref{tab:costs} are such that $n \leq m$). This gap is due to the fact that
interactions along a single session are not affected by other sessions; this, in combination with 
linearity of session types, means that reverting interactions along a single session is like reverting 
a sequential computation. Instead, in the multiple sessions setting, the computation of a session 
can interleave with the computations of others. Thus, in this case reverting a session corresponds to
revert a concurrent computation in a causal-consistent way, which requires to revert interactions
performed along other sessions that have a casual dependence with the interactions of the session 
to be reverted. 
\fi

==> tex/properties.tex <==
% !TEX root = ../reversible_sessions_TR.tex
\section{Properties of the reversible calculus}
\label{sec:properties}

We present in this section some properties of \respi. 
%
These are standard properties of reversible calculi, and therefore we exploit  
terminology, arguments and proof techniques of previous works (in particular, 
\cite{LaneseMS10,DanosK04,CristescuKV13}).
%
As a matter of notation, we will use $\picSet$ and $\respiSet$
to denote the set of \pic\ processes and of \respi\ processes, respectively.
%
Notation $\tuple{\cdot}$ stands for tuples, e.g. $\tuple{h}$ means $h_1,\ldots,h_n$.


\subsection{Correspondence with \pic}

We first show that \respi\ is a conservative extension of the (session-based) \pic.
In fact, as most reversible calculi, \respi\ is only a decoration of its host calculus. 
Such decoration can be erased by means of the \emph{forgetful map} 
$\forgetMap$, which maps \respi\ terms into 
\pic\ ones by simply removing memories, tag annotations and tag restrictions. 

\begin{definition}[Forgetful map]\label{def:forgetfulMap}
The forgetful map $\forgetMap\ :\ \respiSet \rightarrow \picSet$, 
mapping a \respi\ process $M$ into a \pic\ process $P$,
is inductively defined on the structure of $M$ as follows:
$$
\begin{array}{r@{\ }c@{\ }l@{\qquad\qquad}r@{\ }c@{\ }l}
\forget{\ptag{t}P} & = & P
&
\forget{\res{c}N} & = & \res{c}\forget{N}
\\[.1cm]
\forget{\res{t}N} & = & \forget{N}
&
\forget{N_1 \mid N_2} & = & \forget{N_1}\mid\forget{N_2}
\\[.1cm]
\forget{m} & = & \inact
&
\forget{\nil} & = & \inact\\[.1cm]
\end{array}
$$
\end{definition}

To prove the correspondence between \respi\ and \pic, we need the following 
auxiliary lemma relating structural congruence of \respi\ to that of \pic.

\begin{lemma}\label{lem:str_preserved}
Let $M$ and $N$ be two \respi\ processes. If $M \congr N$ then $\forget{M} \congr \forget{N}$.
\end{lemma}
\begin{proof}
We proceed by induction on the derivation of $M \congr N$
(see Appendix~\ref{app:Correspondence}). 
%For most of the laws 
%in Figure~\ref{fig:congruence_respi} the conclusion is trivial because 
%$\forget{M} \congr \forget{N}$ directly corresponds to a law for \pic\ in Figure~\ref{fig:congruence_pic}.
%Instead, for the eighth and twelve laws, we easily conclude because by applying $\forgetMap$
%we obtain the identity. 
\end{proof}

Now, we can show that each forward reduction of a \respi\ process corresponds to 
a reduction of the corresponding \pic\ process.

\begin{lemma}\label{lem:correspondence}
Let $M$ and $N$ be two \respi\ processes. If $M \fwred N$ then $\forget{M} \red \forget{N}$.
\end{lemma}
\begin{proof}
We proceed by induction on the derivation of $M \fwred N$ (see Appendix~\ref{app:Correspondence}). 
%Base cases:
%\begin{itemize}
%\item \rulelabel{fwCon}: We have that 
%$M \ = \ \ptag{t_1}\requestAct{a}{x}{P_1}\ \mid \ \ptag{t_2}\acceptAct{a}{y}{P_2}$
%\ \ and \ \ 
%$N \ = \ \res{s,t_1',t_2'}(
%	\ptag{t_1'}P_1\subst{\ce{s}}{x} \mid \ptag{t_2'}P_2\subst{s}{y}
%	\mid \amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'})$
%with $s,\ce{s} \notin \freese{P_1,P_2}$. By definition of $\forgetMap$, we obtain
%$\forget{M} \ = \ \requestAct{a}{x}{P_1}\ \mid \ \acceptAct{a}{y}{P_2}$.
%Now, by applying rules \rulelabel{Con} and \rulelabel{Str}, we have
%$\forget{M} \red \res{s}(P_1\subst{\ce{s}}{x} \mid P_2\subst{s}{y} \mid \inact)\ =\ P$.
%By definition of $\forgetMap$, we have $\forget{N}=P$ that permits to conclude.
%\item \rulelabel{fwCom},\rulelabel{fwLab},\rulelabel{fwIf1},\rulelabel{fwIf2}: 
%These cases are similar to the previous one.
%\end{itemize}
%Inductive cases:
%\begin{itemize}
%\item \rulelabel{fwPar}: We have that 
%$M \ = \ M_1 \mid \ M_2$
%\ \ and \ \
%$N \ = \ M_1' \mid \ M_2$.
%By the premise of rule \rulelabel{fwPar}, we also have $M_1 \ \fwred\ M_1'$ from which, 
%by induction, we obtain
%$\forget{M_1} \ \red\ \forget{M_1'}$.
%By definition of $\forgetMap$, we get
%$\forget{M}\ = \ \forget{M_1} \mid \ \forget{M_2}$.
%By applying rule \rulelabel{Par}, we have
%$\forget{M} \red \forget{M_1'} \mid \ \forget{M_2} \ =\ P$.
%Thus, by definition of $\forgetMap$, we have
%$\forget{N} \ = \ P$ that directly permits concluding.
%\item \rulelabel{fwRes}: 
%This case is similar to the previous one; in particular, when the restricted name is a tag, 
%it is not even necessary to apply rule \rulelabel{Res}, because the forgetful map erases 
%the restriction.
%\item \rulelabel{fwStr}: 
%By the premise of rule \rulelabel{fwStr}, we have 
%$M  \congr M'$,
%$M' \fwred N'$
%and $N'  \congr N$.
%By induction, we obtain
%$\forget{M'} \red \forget{N'}$. 
%By applying Lemma~\ref{lem:str_preserved},
%we have $\forget{M}  \congr \forget{M'}$ and $\forget{N'} \congr \forget{N}$
%that allow us to conclude.
%\end{itemize}
\end{proof}


The correspondence between \respi\ and \pic\ reductions is completed by 
the following lemmas, which intuitively are the inverse of 
Lemma~\ref{lem:str_preserved_inv} and
Lemma~\ref{lem:correspondence_inv}.

\begin{lemma}\label{lem:str_preserved_inv}
Let $P$ and $Q$ be two \pic\ processes. If $P \congr Q$ then for 
any \respi\ process $M$ such that $\forget{M}=P$ there exists a \respi\ process
$N$ such that $\forget{N}=Q$ and $M \congr N$.
\end{lemma}
\begin{proof}
The proof is straightforward (see Appendix~\ref{app:Correspondence}). 
%Indeed, given a \respi\ process $M$ such that $\forget{M}=P$,
%it must have the form $\res{\tuple{t}}(\ptag{t}P \mid \prod_{i\in I}m_i)$ up to $\congr$. Thus, 
%the process $N$, such that $\forget{N}=Q$, can be defined accordingly: 
%$N \congr \res{\tuple{t}}(\ptag{t}Q \mid \prod_{i\in I}m_i)$. Now, we can conclude 
%by exploiting the ninth law in Figure~\ref{fig:congruence_respi}, 
%i.e. $\ptag{t}P \congr \ptag{t}Q$\ \ if $P \congr Q$, and the fact that relation $\congr$ on
%\respi\ processes is a congruence. 
\end{proof}


\begin{lemma}\label{lem:correspondence_inv}
Let $P$ and $Q$ be two \pic\ processes. If $P \red Q$ then 
for any \respi\ process $M$ such that $\forget{M}=P$ there exists a \respi\ process
$N$ such that $\forget{N}=Q$ and $M \fwred N$.
\end{lemma}
\begin{proof}
We proceed by induction on the derivation of $P \red Q$ (see Appendix~\ref{app:Correspondence}). 
%Base cases:
%\begin{itemize}
%\item \rulelabel{Con}: We have that 
%$P \, = \, \requestAct{a}{x}{P_1} \mid \acceptAct{a}{y}{P_2}$
% \ and\ \
%$Q \, = \, \res{s}(P_1\subst{\ce{s}}{x} \mid P_2\subst{s}{y})$ 
%with $s,\ce{s} \notin \freese{P_1,P_2}$.
%Let $M$ be a \respi\ process such that $\forget{M}=P$, it must have the form 
%$\res{\tuple{t}}(\ptag{t_1}\requestAct{a}{x}{P_1} \mid \ptag{t_2}\acceptAct{a}{y}{P_2} \mid \prod_{i\in I}m_i)$ up to $\congr$. Thus, by applying rules \rulelabel{fwCon}, \rulelabel{fwPar}, \rulelabel{fwRes} and \rulelabel{fwStr}, 
%we get $M \fwred \res{\tuple{t},s,t_1',t_2'}(
%\ptag{t_1'}P_1\subst{\ce{s}}{x} \mid \ptag{t_2'}P_2\subst{s}{y}
%\mid \amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'} \mid \prod_{i\in I}m_i) \, =\, N$.
%We conclude by applying $\forgetMap$ to $N$, since we obtain $\forget{N}=Q$.
%\item \rulelabel{Com},\rulelabel{Lab},\rulelabel{If1},\rulelabel{If2}: 
%These cases are similar to the previous one.
%\end{itemize}
%Inductive cases:
%\begin{itemize}
%\item \rulelabel{Par}: We have that 
%$P \ = \ P_1 \mid P_2$
%\ \ and \ \
%$Q \ = \ P_1' \mid P_2$.
%Let $M$ be a \respi\ process such that $\forget{M}=P_1 \mid P_2$. 
%We have $M \congr \res{\tuple{t}}(\ptag{t_1}P_1 \mid \ptag{t_2}P_2 \mid  \prod_{i\in I}m_i)
%\congr \res{\tuple{t'}}(M_1 \mid \ptag{t_2}P_2 \mid  \prod_{j\in J}m_j)$
%with $M_1\congr  \res{\tuple{t''}}(\ptag{t_1}P_1 \mid \prod_{k\in K}m_k)$,
%$\tuple{t}=\tuple{t'},\tuple{t''}$ and $J\cup K=I$.
%By the premise of rule \rulelabel{Par}, we also have $P_1 \red P_1'$ from which, 
%by induction, since $\forget{M_1}=P_1$, 
%there exists $M_1'$ such that $\forget{M_1'}=P_1'$ and $M_1 \fwred M_1'$.
%Thus, by applying rules \rulelabel{fwPar}, \rulelabel{fwRes} and \rulelabel{fwStr}, 
%we get 
%$M \fwred  \res{\tuple{t'}}(M_1' \mid \ptag{t_2}P_2 \mid  \prod_{j\in J}m_j)\,=\,N$.
%We conclude by applying $\forgetMap$ to $N$, because
%$\forget{N}=\forget{M_1'} \mid P_2= P_1' \mid P_2 =Q$.
%\item \rulelabel{Res}: 
%This case is similar to the previous one.
%\item \rulelabel{Str}: We have that 
%$P \congr P'$, $Q \congr Q'$ and $P' \red Q'$.
%Let $M$ be a process such that $\forget{M}=P$.
%By applying Lemma~\ref{lem:str_preserved_inv}, 
%there exists $M'$ such that $\forget{M'}=P'$ and $M \congr M'$.
%By induction, there is $N'$ such that $\forget{N'}=Q'$ and $M' \fwred N'$.
%By applying Lemma~\ref{lem:str_preserved_inv} again, 
%there exists $N$ such that $\forget{N}=Q$ and $N \congr N'$.
%By applying rule \rulelabel{fwStr}, we conclude $M \fwred N$.
%\end{itemize}
\end{proof}





\subsection{Loop lemma}
The following lemma shows that in \respi\ backward reductions are the inverse 
of the forward ones and vice versa.  Notice that we are considering here only 
reachable processes. 

\begin{lemma}[Loop lemma]\label{lemma:loop}
Let $M$ and $N$ be two reachable \respi\ processes. 
$M \fwred N$ if and only if $N \bwred M$.
\end{lemma}
\begin{proof}
The proof for the \emph{if} part is by induction on the derivation of $M \fwred N$, %.
%Base cases:
%\begin{itemize}
%\item \rulelabel{fwCon}: We have that 
%$M \ = \ \ptag{t_1}\requestAct{a}{x}{P_1}\ \mid \ \ptag{t_2}\acceptAct{a}{y}{P_2}$
%\ \ and \ \ 
%$N \ = \ \res{s,t_1',t_2'}(
%	\ptag{t_1'}P_1\subst{\ce{s}}{x} \mid \ptag{t_2'}P_2\subst{s}{y}
%	\mid \amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'})$
%with $s,\ce{s} \notin \freese{P_1,P_2}$. 
%By applying rule \rulelabel{bwCon}, we can directly conclude 
%$N \bwred M$.
%\item \rulelabel{fwCom},\rulelabel{fwLab},\rulelabel{fwIf1},\rulelabel{fwIf2}: 
%These cases are similar to the previous one.
%\end{itemize}
%Inductive cases:
%\begin{itemize}
%\item \rulelabel{fwPar}: We have that 
%$M  =  N_1 \mid N_2$, $N  = N_1' \mid N_2$ and $N_1 \fwred N_1'$.
%By induction $N_1' \bwred N_1$. Thus, we conclude by applying rule \rulelabel{bwPar},
%since we get $N  = N_1' \mid N_2 \bwred N_1 \mid N_2 = M$.
%\item \rulelabel{fwRes} and \rulelabel{fwStr}: 
%These cases can be proved by straightforwardly resorting to the induction hypothesis as in the previous case.
%\end{itemize}
%
%\noindent
%The proof for the \emph{only if} part is by induction on the derivation of $N \bwred M$.
while the proof for the \emph{only if} part is by induction on the derivation of $N \bwred M$
(see Appendix~\ref{app:LoopLemma}).
%Base cases:
%\begin{itemize}
%\item \rulelabel{bwCon}: We have that 
%$N \ = \ \res{s,t_1',t_2'}(\ptag{t_1'}P \mid \ptag{t_2'}Q 
%	\mid \amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'})$
%\ \ and \ \ 
%$M \ = \ \ptag{t_1}\requestAct{a}{x}{P_1}\ \mid \ \ptag{t_2}\acceptAct{a}{y}{P_2}$.
%Since $N$ is a reachable process, memory $\amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'}$
%has been generated by a synchronisation between threads
%$\ptag{t_1}\requestAct{a}{x}{P_1}$ and $\ptag{t_2}\acceptAct{a}{y}{P_2}$,
%producing a session channel $s$ and two continuation processes 
%$P_1\subst{\ce{s}}{x}$ and $P_2\subst{s}{y}$ tagged by $t_1'$ and $t_2'$, respectively.
%Now, by tag uniqueness implied by reachability and use of restriction in tag generation,
%$P$ and $Q$ must coincide with $P_1\subst{\ce{s}}{x}$ and $P_2\subst{s}{y}$, respectively.
%Therefore, by applying rule \rulelabel{fwCon}, we can directly conclude $M \fwred N$.
%\item \rulelabel{bwCom},\rulelabel{bwLab},\rulelabel{bwIf}: 
%These cases are similar to the previous one.
%\end{itemize}
%Inductive cases:
%\begin{itemize}
%\item \rulelabel{bwPar}: We have that 
%$N  =  N_1 \mid N_2$, $M  = N_1' \mid N_2$ and $N_1 \bwred N_1'$.
%By induction $N_1' \fwred N_1$. Thus, we conclude by applying rule \rulelabel{fwPar},
%since we get $M  = N_1' \mid N_2 \fwred N_1 \mid N_2 = N$.
%\item \rulelabel{bwRes} and \rulelabel{bwStr}: 
%These cases can be proved by straightforwardly resorting to the induction hypothesis as in the previous case.
%\end{itemize}
\end{proof}



\subsection{Causality}

We show here that reversibility in \respi\ is causally consistent. 

As in \cite{LaneseMS10} and \cite{DanosK04}, we rely on the notion of transition.
%
A \emph{transition} is a triplet of the form \mbox{$M \transition{m,\mSet,\fwred} N$}
(resp. \mbox{$M \transition{m,\mSet,\bwred} N$}), where 
$M$ and $N$ are closed reachable \respi\ processes such that
$M \fwred N$ (resp. $M \bwred N$), 
$m$ is the action or choice memory involved in the reduction, 
and $\mSet$ is the set of fork memories possibly involved in the reduction.
%
A memory is \emph{involved in} a reduction if it is created or removed by the reduction.
%
We use $\tlab$ to denote transition \emph{labels} $(m,\mSet,\fwred)$ and $(m,\mSet,\bwred)$.
If $\tlab$ is $(m,\mSet,\fwred)$, then its inverse is $\inver{\tlab}=(m,\mSet,\bwred)$
and vice versa. 
%
In a transition $M \transition{\tlab} N$, we call $M$ the \emph{source} of the transition 
and $N$ its \emph{target}. We use $\tName$ to range over transitions; $\inver{\tName}$
denotes the inverse of transition $\tName$.

Two transitions are \emph{coinitial} if they have the same source, 
\emph{cofinal} if they have the same target, \emph{composable} if the 
target of one is the source of the other. 
A sequence of pairwise composable transitions is called a \emph{trace};
we use $\trace$ to range over traces.
Notions of target, source and composability extend naturally to traces.
We use $\emptytrace{M}$ to denote the empty trace with source $M$
and $\trace_1;\trace_2$ the composition of two composable traces $\trace_1$
and $\trace_2$.

We only consider only transitions $M \transition{\tlab} N$ where $M$ and $N$ 
do not contain threads of the $\ptag{t}(P\mid Q)$.
This condition can be always satisfied by splitting all such kind of threads into 
sub-threads, until their disappearance in the considered terms, using structural
law $\ptag{t}(P\mid Q) \congr \res{t_1,t_2}(\ptag{t_1}P \mid \ptag{t_2}Q \mid \fmem{\fev{t}{t_1}{t_2}})$. 
Moreover, since conflicts between transitions are identified by means of tag identifiers
(see Definition~\ref{def:concurrentTrasitions} below), we only consider transitions
that do not use $\alpha$-conversion on tags, and that generates fork memories in a 
deterministic way, e.g. given a memory $\fmem{\fev{t}{t_1}{t_2}}$ tags $t_1$ and $t_2$
are generated by applying an injective function to $t$.

The \emph{stamp} $\stamp{\tlab}$ of a transition label $\tlab$ identifies the threads
involved in the corresponding transition, and is defined as follows (we use $\tagSet$
to denote a set of tags $\{t_i\}_{i \in I}$):
$$
\begin{array}{l}
\stamp{m,\mSet,\fwred} = \stamp{m,\mSet,\bwred} = \stamp{m}\cup\stampFork{\stamp{m}}{\mSet}
\\[.3cm]
\stamp{\amem{\actEv{t_1}{\storedAct}{t_2}}{t_1'}{t_2'}} = \set{t_1,t_2,t_1',t_2'}
\\[.3cm]
\stamp{\cmem{t}{\ifEv{e}{P}{Q}}{t'}} = \set{t,t'}
\\[.3cm]
\stampFork{\tagSet}{\set{m_i}_{i \in I}} = \bigcup_{i\in I}\stampFork{\tagSet}{m_i}
\\[.3cm]
\stampFork{\tagSet}{\fmem{\fev{t}{t_1}{t_2}}} = \left\{
\begin{array}{@{}ll}
\set{t_1,t_2} & \text{if } t\in \tagSet\\[.1cm]
\emptyset & \text{otherwise}
\end{array}\right.
\end{array}
$$
The stamp of fork memories permits to take into account 
the relationships between a thread and its sub-threads.
This is similar to the closure over tags used in \cite{GLMT}.
Notably, as in \cite{LaneseMS10}, the tags of 
continuation processes are inserted into a stamp, in order to 
take into account possible conflicts between a forward 
transition and a backward one.  
Notice also that it is instead not necessary include 
in the stamp the fresh session channel created or used
by a reduction. In fact, this would be useful to detect conflicts
between the transitions involving the memory corresponding to
the creation of the channel and the transitions where such channel 
is used. However, such conflicts are already implicitly considered,
since after the creation the channel is only known by the threads 
corresponding to the continuation processes, which are already 
considered in the stamp as discussed above.

We can now define when two transitions are concurrent.
\begin{definition}[Concurrent transitions]\label{def:concurrentTrasitions}
Two coinitial transitions $M \transition{\tlab_1} M_1$
and $M \transition{\tlab_2} M_2$ are \emph{in conflict} if 
%\vspace*{-.5cm}
\begin{itemize}
\item $\exists\ t \in \stamp{\tlab_1}$ such that $t \in \stamp{\tlab_2}$, or
\item $\exists\ t \in \stamp{\tlab_2}$ such that $t \in \stamp{\tlab_1}$.
\end{itemize}
Two coinitial transitions are \emph{concurrent} if they are not in conflict.  
\end{definition}

The following lemma characterises the causally independence among
concurrent transitions.

\begin{lemma}[Square lemma]
If $\tName_1=M\transition{\tlab_1}M_1$ and $\tName_2=M\transition{\tlab_2}M_2$
are two coinitial concurrent transitions, then there exist two cofinal transitions
$\tName_2/\tName_1=M_1\transition{\tlab_2}N$ and $\tName_1/\tName_2=M_2\transition{\tlab_1}N$.
\end{lemma}
\begin{proof} %\emph{(Sketch)}\ \
By case analysis on the form of transitions $\tName_1$ and $\tName_2$.
\end{proof}

In order to study the causality of \respi\ reversibility, we introduce the notion 
of \emph{causal equivalence} between traces, denoted $\causallyEq$.
This is defined as the least equivalence relation between traces closed under 
composition that obeys the following rules:
$$
\tName_1\,;\,\tName_2/\tName_1 \ \causallyEq \ \tName_2\,;\,\tName_1/\tName_2
\qquad\qquad
\tName\,;\,\inver{\tName} \ \causallyEq\ \emptytrace{\source{\tName}}
\qquad\qquad
\inver{\tName}\,;\,\tName \ \causallyEq\ \emptytrace{\target{\tName}}
$$
Intuitively, the first rule states that the of execution order of two concurrent transitions
can be swapped, while the other rules state that the composition of a trace with its inverse 
is equivalent to the empty transition.
 
Now, we conclude with the result stating that two coinitial causally equivalent traces  
lead to the same final state. Thus, in such case, we can rollback to the initial state by 
reversing any of the two traces. 

\begin{theorem}[Causal consistency]
Let $\trace_1$ and $\trace_2$ be coinitial traces. Then, $\trace_1 \causallyEq \trace_2$
if and only if $\trace_1$ and $\trace_2$ are cofinal. 
\end{theorem}
\begin{proof}\emph{(Sketch)}\ \
By construction of $\causallyEq$, if $\trace_1 \causallyEq \trace_2$ then 
$\trace_1$ and $\trace_2$ must be coinitial and cofinal, so this direction of the theorem 
is verified. 
%
The proof that $\trace_1$ and $\trace_2$ being coinitial and cofinal implies that 
$\trace_1 \causallyEq \trace_2$ is based on a lemma (Rearranging Lemma),
which permits expressing the two traces as composition of a backward trace 
and a forward one, and proceed by lexicographic induction on the sum of the 
lengths of $\trace_1$ and $\trace_2$ and on the distance between the end of 
$\trace_1$ and the earliest pair of transitions, one  in $\trace_1$ and another in $\trace_2$, 
that are not equal. 
\end{proof}


==> tex/relatedWork.tex <==
% !TEX root = ../reversible_sessions_TR.tex
\section{Related work}
\label{sect:relatedWork}
Our proposal combines the notion of (causal-consistent) reversibility with (typed) primitives supporting session-based interactions in concurrent systems. Therefore, below, we review some of the closely related works concerning either reversibility or session types.

Despite being a subject of study since many years, reversible computing is recently experiencing a rise in popularity. This is mainly due to the fact that reversibility is a key ingredient in different application domains, e.g. biological systems, hardware design, quantum computing, software debugging and --for what specifically concerns our study--  design of reliable concurrent systems.
%
Thus, considered the subject of our work, the most closely related works in the reversible computing field concern the definition of \emph{reversible process calculi}. 
%
In Table~\ref{tab:relWork}, we classify the main reversible calculi proposed so far in the literature according to the formalisms they are based on (namely, CCS \cite{CCS}, \pic~\cite{PICALC} and DSD~\cite{CardelliL09}) and according to the key instruments they exploit to achieve reversibility. 

\begin{table}[t]
\caption{Reversible process calculi classification} 
\vspace*{-.2cm}
	\begin{centering}	
		\begin{tabular}{|r||c|c|c|c|c|}
		\hline
		& \textbf{Formalism} 
		& \textbf{Memories} 
		&\textbf{Identifiers} 
		& \textbf{Fork handling} 
		& \textbf{Semantics}
		\\
		\hline
		\hline
		RCCS~\cite{DanosK04} & CCS & memory stacks & %memories as ids 
		memories& fork numbers  & labelled \\
		\hline
		CCS-R~\cite{DanosK07a} & CCS & memory stacks & thread ids & empty memories & labelled \\
		\hline
		CCSK~\cite{PhillipsU07} & CCS & \multicolumn{1}{c|}{--} & %communication 
		communic.& \multicolumn{1}{c|}{--} & labelled\\
		& & \multicolumn{1}{c|}{\small (static-like rules)} & keys &&\\
		\hline
		$\rho\pi$~\cite{LaneseMS10} & \pic & non-structured &  thread ids & structured tags & reduction\\
		& & memories &&&\\
		\hline
		R$\pi$~\cite{CristescuKV13} & \pic & memory stacks & event ids & fork symbol & labelled\\
		\hline
		Reversible  & DSD & \multicolumn{1}{c|}{--}  & signal ids & \multicolumn{1}{c|}{--} & reduction\\	
		structures~\cite{CardelliL11} & & \multicolumn{1}{c|}{{\small(pointers to}} & & & \\ 
		& & \multicolumn{1}{c|}{{\small next operations)}} &&&\\
		\hline
		\end{tabular}
		\label{tab:relWork}
		\vspace*{-.4cm}
	\end{centering}
\end{table}

Reversible CCS (RCCS)~\cite{DanosK04} is the first proposal of reversible calculus, from which all subsequent 
works drew inspiration. The host calculus is CCS without recursive definitions and relabelling. 
%
To each currently running thread is associated an individual memory stack keeping track 
of past actions, as well as forks and synchronisations. Information pushed on the memory stacks,
upon doing a forward transition, can be then used for a roll-back.
%
The memories also serve as a naming scheme and yield unique identifiers for threads.
%
When a process divides in two sub-threads, each sub-thread inherits the father memory together 
with a fork number (either $\langle 1 \rangle$ or $\langle 2 \rangle$) indicating which of the two 
sons the thread is. Then, in case of a forward synchronisation, the synchronised threads exchange
their names (i.e., memories) in order to allows the corresponding backward synchronisation to 
take place. A drawback of this approach for memorising fork actions is that the parallel operator 
does not satisfy usual structural congruence rules as commutativity, associativity and 
nil process as neutral element. It is proved that RCCS is causally consistent, i.e. the calculus 
allows backtrack along any causally equivalent past, where concurrent actions can be swapped and 
successive inverse actions can be cancelled. RCCS has been used for studying a general notion
of transactions in \cite{DanosK05}.

CCS-R~\cite{DanosK07a} is another reversible variant of CCS,
which however mainly aims at formalising biological systems.  
%
Like the previous calculus, it relies on memory stacks for storing information needed for 
backtracking, which now also record events corresponding to the unfolding of process 
definitions. Instead, differently from RCCS, specific identifiers are used to label threads;
in case of unfolding, sub-threads are labelled on-the-fly. Moreover, forking now does not 
exploit fork numbers, but it requires the memory stack of a given thread be empty before enabling 
the execution of its sons; this forces the sub-threads to share the memory that their father
had before the forking. As in RCCS, in case of synchronisation, the communicating threads 
exchange their identifiers. The transition system of CCS-R is proved to be reversible and it 
is demonstrated that CCS-R is sound and complete w.r.t. CCS.

CCS with communication Keys (CCSK)~\cite{PhillipsU07} is a reversible process calculus
obtained by applying a general procedure to produce reversible calculi.
%
A relevant aspect of this approach is that it does not rely on memories for supporting backtracking. 
The idea is to maintain the structure of processes fixed throughout computations, thus
avoiding to consume guards and alternative choices, which is the source of irreversibility.
Past behaviour and discarded alternatives are then recorded in the syntax of terms.
This is realised by transforming the dynamic rules of the SOS semantics into static-like rules.
In this way, backward rules are obtained simply as symmetric versions of the forward rules.
%
Moreover, to ensure that synchronisations are properly reverted, two communicating threads have to 
agree on a communication key, which will uniquely identify that communication. In this
way, the synchronising actions are locked together and can only be undone together. 
%
As usual, results showing that the method yields well-behaved transition relations are provided.
%
The proposed converting procedure can be applied to other calculi without name passing, 
such as ACP~\cite{BergstraK84} or CSP~\cite{BrookesHR84},
but it is not suitable for calculi with name binders, as \pic, which we are interested in this work.

$\rho\pi$~\cite{LaneseMS10} is a reversible variant of the higher-order \pic.
It borrows from RCCS the use of memories for keeping track of past actions, 
although in $\rho\pi$ memories are not stacks syntactically associated to threads,
but they simply are terms, each one dedicated to a single communication, in parallel with 
processes. The connection between memories and threads is kept by resorting to 
identifiers in a way similar to CCSK. However, in $\rho\pi$, to properly handling forking, 
specific structured tags are used to connect the identifier of the father thread with 
the identifiers of its sub-threads. 
%
Besides proving that $\rho\pi$ is casually consistent, it is also shown that it can be
faithfully encoded into higher-order \pic.
%
Notably, differently from the approaches mentioned before,
the semantics of $\rho\pi$ is given in a reduction style. 
%
A variant of this calculus, called $\mathsf{roll}\mathrm{-}\pi$~\cite{LaneseMSS11}, has been defined 
to control backward computations by means of a roll-back primitive.  
%
Moreover, the approaches proposed in \cite{LaneseMS10,LaneseMSS11} have been 
applied in \cite{GLMT} for reversing a variant of Klaim~\cite{NicolaFP98}.

Another reversible variant of \pic\ is R$\pi$~\cite{CristescuKV13}. 
Differently from $\rho\pi$, R$\pi$ considers as host calculus a standard \pic\ (without choice and 
replication) and its semantics is defined in terms of a labelled transition relation. 
This latter point requires to introduce some technicalities to properly deal with scope extrusion. 
Similarly to RCCS,  this calculus relies on memory stacks, now recording events (i.e., consumed 
prefixes and related substitutions) and forking (by means of the fork symbol $\langle \uparrow \rangle$).
%
Results about the notion of causality induced by the semantics of the calculus are provided.

Finally, reversible structures~\cite{CardelliL11} is a simple computational calculus for modelling
chemical systems. Since such systems are naturally reversible but have no backtracking memory, 
differently from most of the above proposals, reversible structures does not exploit memories but 
maintains the structure of terms and uses a special symbol $\,\hat{}\,$ to indicate the next operations 
(one forward and one backward) that a term can perform. Terms of the calculus are parallel compositions 
of signals and gates (i.e., terms that accept input signals and emit output signals), which interact 
according to a CCS-style model. When a forward synchronisation takes place, the executed gate input
is labelled by the identifier of the consumed signal, and the pointer symbol inside the gate is moved 
forward. The backwards computation is realised by executing these operations in a reverse way, thus 
releasing the output signal. As usual, the interplay between casual dependency and reversible structures
is studied, with the novelty that in this setting signal identifiers are not necessary unique.  

% OTHER RELATED WORK ON REVERSIBILITY
% We could cite other works on reversibility based on event structures. But they are less related to our works.

In our work we mainly take inspiration from the $\rho\pi$ approach. 
In fact, all other approach based on CCS and DSD cannot be 
directly applied to a calculus with name-passing. Moreover, the $\rho\pi$ approach is 
preferable to the R$\pi$ one because the former proposes a reduction semantics, in which we are 
interested in, while the latter proposes a labelled semantics, which would complicate our theoretical
framework (in order to properly deal with scope extension of names). More specifically, 
we use unique (non-structured) tags for identifying threads and memories for recording 
taking place of actions, choices and forking. Each memory is devoted to store the information
needed to revert a single event, and memories are connected each other, in order to keep track 
of computation history, by using tags as links.

For what concerns the related works on session-based calculi, it is worth noticing that we
decided to consider a setting more standard and simpler as possible, which is that with 
synchronous binary sessions. In particular, our host calculus is the variant of \pic\ 
introduced in \cite{YoshidaV07}, whose notation has been revised according to \cite{MostrousY09}.
We leave for future investigation the application of our approach to formalisms relying on the
other forms of sessions introduced in the literature, among which we would like to mention
asynchronous binary sessions~\cite{CoppoDY07},
multiparty asynchronous sessions~\cite{HondaYC08},
multiparty synchronous sessions~\cite{BejleriY09},
sessions with higher-order communication~\cite{MostrousY09},
sessions specifically devised for service-oriented computing~\cite{BorealeBNL08,BruniLMT08,CairesV10}.

%Finally, for what concerns the specific contribution of this work, as far as we know this is 
%the first attempt of combining reversibility and session-based interaction. 

==> tex/reversible_calculus.tex <==
% !TEX root = ../reversible_sessions_TR.tex
\section{Reversible Session-based \pic}
\label{sec:rev_calculus}

In this section, we introduce a reversible extension of the 
calculus described in Section~\ref{sec:host_calculus}.
%
We call \respi\ (\emph{Reversible Session-based} $\pi$) such calculus.
 
As explained in Section~\ref{sect:relatedWork}, a reversible calculus 
is typically obtained from the corresponding host calculus by adding 
memory devices to store information about interactions and their effects 
on the system, which otherwise would be lost during forward computations.
In doing this, we follow the approach of~\cite{LaneseMS10}, which in its 
turn is inspired by~\cite{DanosK04} (for the use of memories) and 
by~\cite{PhillipsU07} (for the use of thread identifiers). 
Of course, since here we consider as host calculus a session-based variant 
of standard \pic\ rather than an asynchronous higher-order variant, the 
technical development is different. 

Roughly, our approach to keep track of computation history is as follows: 
we tag processes with unique identifiers and use memories to store the 
information needed to reverse each single forward reduction. Thus, 
the history of a reduction sequence is stored in a number of small memories 
connected each other by using tags as links.  
%
In this way, \respi\ terms can perform, besides \emph{forward computations}
(denoted by $\fwred$), also  \emph{backward computations} (denoted by $\bwred$)
that undo the effect of the former ones. Like all other formalisms for reversible computing 
in concurrent settings, forward computations are undone in a \emph{causal-consistent} 
fashion, i.e. backtracking does not have to necessarily follow the exact order of forward 
computations in reverse, since independent (more precisely, \emph{concurrent})
actions can be undone in a different order. Thus, an action can be undone only 
after all the actions causally depending on it have already been undone.
%
We will come back on causal-consistency in Section~\ref{sec:properties}.



\subsection{Syntax}
The syntax of \respi\ is given in Figure~\ref{fig:syntax_respi}.
In addition to the base sets used for \pic\ processes in Section~\ref{sec:host_calculus},
here we use \emph{tags}, ranged over by $t$, $t'$, \ldots, to uniquely identify \emph{threads}.
Letters $h$, $h'$, \ldots denote \emph{names}, i.e. 
(shared and session) channels and tags together. 
Uniqueness of tags is ensured by using the restriction operator and by 
only considering \emph{reachable} terms (see Definition~\ref{def:reachable}).

\respi\ processes are built upon standard (session-based) \pic\ processes by labelling them 
with tags. Thus, the syntax of  \pic\ processes $P$, as well as of expressions $e$,
is that same of that shown in Figure~\ref{fig:syntax_pi} and, hence, it is omitted here.
It is worth noticing that only \respi\ processes can execute (i.e., \pic\ ones cannot
directly evolve).

\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{rcl@{\hspace{-.5cm}}r}
	\textbf{\respi\ Processes}\quad
	$M$ & ::= & $\ptag{t}P$ & thread\\
	& $\mid$ & $\res{h}\, M$ & channel/tag restriction\\		
	& $\mid$ & $M \mid N$ & parallel composition\\	
	& $\mid$ & $m$ & memory\\
	& $\mid$ & $\nil$ & empty process\\	
	\\	
	\textbf{Memories}\quad	
	$m$ & ::= & $\amem{\actEv{t_1}{\storedAct}{t_2}}{t_1'}{t_2'}$ & action memory\\
	& $\mid$ & $\cmem{t}{\ifEv{e}{P}{Q}}{t'}$ & choice memory\\
	& $\mid$ & $\fmem{\fev{t}{t_1}{t_2}}$ & fork memory\\
	\\[-.2cm]
	$\storedAct$ & ::= & 	$\initAct{a}{x}{y}{P}{Q}{s}$ 
	\ \ $\mid$ \ \ $\comAct{k}{e}{x}{P}{Q}$ 
	& action events\\
	& $\mid$ & $\selAct{k}{l_i}{P}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$ & \\	 
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{\respi\ syntax (\pic\ Processes $P$ and Expressions $e$ are in Figure~\ref{fig:syntax_pi})}
	\label{fig:syntax_respi}
	%\vspace*{.4cm}
	\end{centering}
\end{figure}

Moreover, \respi\ extends \pic\ with \emph{memory} processes $m$. In particular, 
there are three kind of memories: 
\begin{itemize}
\item \emph{Action memory} $\amem{\actEv{t_1}{\storedAct}{t_2}}{t_1'}{t_2'}$, 
storing an action event $\storedAct$ together with the tag $t_1$
of the active party of the action, the tag $t_2$ of the corresponding 
passive party, and the tags $t_1'$ and $t_2'$ of the two new threads activated by the 
corresponding reduction.
%
An \emph{action event} $\storedAct$, as we shall clarify later, records all information 
necessary to revert the correspond interaction, which can be either a session initiation
$\initAct{a}{x}{y}{P}{Q}{s}$, 
a communication along an established session $\comAct{k}{e}{x}{P}{Q}$, 
or a branch selection $\selAct{k}{l_i}{P}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$.
Notably, in the latter two events, $k$ can only be either $s$ or $\ce{s}$ (i.e., it cannot be a variable).

\item \emph{Choice memory} $\cmem{t}{\ifEv{e}{P}{Q}}{t'}$, storing a choice event $\ifEv{e}{P}{Q}$
together with the tag $t$ of the conditional choice and the tag $t'$ of the new activated thread.
The choice event $\ifEv{e}{P}{Q}$ records the evaluated expression $e$, 
and the processes $P$ and $Q$ of the then-branch and else-branch, respectively.

\item \emph{Fork memory} $\fmem{\fev{t}{t_1}{t_2}}$, storing the tag $t$ of a splitting 
thread, i.e. a thread of the form $\ptag{t}(P\mid Q)$, together with the tags $t_1$ and $t_2$
of the two new activated threads, i.e. $\ptag{t_1}P$ and $\ptag{t_2}Q$.
The use of fork memories is analogous to that of \emph{connectors} in \cite{GLMT}. 
\end{itemize}


Threads and memories are composed by parallel composition and restriction operators.
The latter, as well as notion of bound and free identifiers, extend to names.  
%
In particular, for $M$ a \respi\ process, 
$\freet{M}$ denotes the set of \emph{free tags}; 
$\freev{\cdot}$, $\freec{\cdot}$ and $\freese{\cdot}$ 
extend naturally to \respi\ processes. 
%
Of course, we still rely on the same assumptions on free and bound variables/channels  
mentioned in Section~\ref{sec:syntax_pic}.
%
Moreover, we need further assumptions in case of \respi\ processes, since not all 
processes allowed by the syntax in Figure~\ref{fig:syntax_respi} are semantically meaningful. 
Indeed, in a general term of the calculus, the history stored in the memories may not be
consistent, due to the use of non-unique tags or broken connections between continuation tags
within memories  and corresponding threads.  
%
For example, given the choice memory $\cmem{t}{\ifEv{e}{P}{Q}}{t'}$,
we have a broken connection when no thread tagged by $t'$ exists in the \respi\ process and 
no memory of the form $\amem{\actEv{t'}{\storedAct}{t_2}}{t_1'}{t_2'}$,
$\amem{\actEv{t_1}{\storedAct}{t'}}{t_1'}{t_2'}$,
$\cmem{t'}{\ifEv{e}{P_1}{P_2}}{t_1}$,
and $\fmem{\fev{t'}{t_1}{t_2}}$
exist.
%
Thus, as in~\cite{CristescuKV13}, to ensure history consistency we only consider \emph{reachable} 
processes, i.e. processes obtained by means of forward and backward reductions from processes
with unique tags and no memory.

\begin{definition}[Reachable processes]\label{def:reachable}
The set of \emph{reachable} \respi\ processes is the closure 
under $\fwbwred$ (see Section~\ref{sec:respi_sem}) of the set of 
%terms generated by the following grammar:
terms, whose threads have distinct tags, generated by the following grammar:
$$
M\ ::= \ \ptag{t}P 
\ \ \mid\ \ 
\res{c}\, M
\ \ \mid\ \ 
M \mid N
\ \ \mid\ \ 
\nil
$$
%and such that, for each term, its threads have distinct tags. 
\end{definition}

\subsection{Semantics}
\label{sec:respi_sem}
The operational semantics of \respi\ is given in terms of a structural congruence and 
of a reduction relation.

The \emph{structural congruence} $\congr$ extends that of \pic\ (Figure~\ref{fig:congruence_pic})
with the additional laws in Figure~\ref{fig:congruence_respi}.
Most of the new laws simply deal with the parallel and restriction operators on \respi\
processes. Thus, we only focus on relevant laws. 
%
The eighth law permits moving a restriction on a \pic\ process to the level of 
\respi\ processes.
%
The ninth law lifts the congruence at \pic\ process level to the threads level. 
%
The last law is crucial for fork handling: it permits splitting a single thread composed of two parallel processes 
into two threads with fresh tags; the tag of the original thread and the new tags are properly recoreded in a 
fork memory. 

%\begin{figure}[t]
%	\begin{centering}
%	\begin{tabular}{@{}l@{\qquad }l@{\qquad}l@{}}
%	$(M \mid N) \mid L \congr M \mid (N \mid L)$ 
%	&
%	$M \mid N \congr N \mid M$ 
%	&
%	$M \mid \nil \congr M$
%	\\[.3cm]
%	$\res{t}M \mid N \congr \res{t}(M \mid N)$\ \ if $t \notin \freet{N}$
%	&
%	$\res{h_1}\res{h_2}M \congr \res{h_2}\res{h_1}M$
%	&
%	$\res{h}\, \nil \congr \nil$
%	\\[.3cm]
%	$\res{a}M \mid N \congr \res{a}(M \mid N)$\ \ if $a \notin \freec{N}$
%	&
%	$\ptag{t}\res{c}P \congr \res{c}\,\ptag{t}P$
%	&
%	$\ptag{t}P \congr \ptag{t}Q$\ \ if $P \congr Q$
%	\\[.3cm]
%	$\res{s}M \mid N \congr \res{s}(M \mid N)$\ \ if $s,\ce{s} \notin \freese{N}$
%	&
%	$M \congr N$\ \ if $M \alphaeq N$
%	&
%	\\[.3cm]
%	\multicolumn{3}{@{}l@{}}{
%	$\ptag{t}(P\mid Q) \congr \res{t_1,t_2}(\ptag{t_1}P \mid \ptag{t_2}Q \mid \fmem{\fev{t}{t_1}{t_2}})$}
%	\\[.2cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.3cm}
%	\caption{\respi\ structural congruence (additional laws)}
%	\label{fig:congruence_respi}
%	%\vspace*{.3cm}
%	\end{centering}
%\end{figure}
\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{l@{\qquad }l}
	$(M \mid N) \mid L \congr M \mid (N \mid L)$ 
	&
	$M \mid N \congr N \mid M$ 
	\\[.3cm]
	$M \mid \nil \congr M$
	&
	$\res{h}\, \nil \congr \nil$
	\\[.3cm]
	$\res{t}M \mid N \congr \res{t}(M \mid N)$\ \ if $t \notin \freet{N}$
	&
	$\res{h_1}\res{h_2}M \congr \res{h_2}\res{h_1}M$
	\\[.3cm]
	$\res{a}M \mid N \congr \res{a}(M \mid N)$\ \ if $a \notin \freec{N}$
	&
	$\ptag{t}\res{c}P \congr \res{c}\,\ptag{t}P$
	\\[.3cm]	
	$\ptag{t}P \congr \ptag{t}Q$\ \ if $P \congr Q$
	&
	$\res{s}M \mid N \congr \res{s}(M \mid N)$\ \ if $s,\ce{s} \notin \freese{N}$
	\\[.3cm]	
	$M \congr N$\ \ if $M \alphaeq N$
	&
	\\[.3cm]
	\multicolumn{2}{@{}l@{}}{
	$\ptag{t}(P\mid Q) \congr \res{t_1,t_2}(\ptag{t_1}P \mid \ptag{t_2}Q \mid \fmem{\fev{t}{t_1}{t_2}})$}
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}
	\caption{\respi\ structural congruence (additional laws)}
	\label{fig:congruence_respi}
	%\vspace*{.3cm}
	\end{centering}
\end{figure}



The \emph{reduction relation} of \respi, written $\fwbwred$, is given as the union 
of the forward and backward reduction relations defined by the rules in 
Figure~\ref{fig:reduction_respi}: $\fwbwred\ = \ \fwred \cup \bwred$.
As usual, $\fwred$ and $\bwred$ are the smallest relations on 
closed \respi\ processes generated by the corresponding rules in the figure.

%\begin{figure}[t]
%	\begin{centering}
%	\begin{tabular}{@{}l@{\ }l@{\quad}l@{}}
%	$\ptag{t_1}\requestAct{a}{x}{P_1}\ \mid \ \ptag{t_2}\acceptAct{a}{y}{P_2}$
%	& $s,\ce{s} \notin \freese{P_1,P_2}$ &\rulelabel{fwCon}
%	\\[.1cm]
%	\quad $\fwred\ \  \res{s,t_1',t_2'}(
%	\ptag{t_1'}P_1\subst{\ce{s}}{x} \mid \ptag{t_2'}P_2\subst{s}{y}
%	\mid \amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'})$
%	\\[.3cm]
%	$\res{s,t_1',t_2'}(\ptag{t_1'}P \mid \ptag{t_2'}Q 
%	\mid \amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'})$
%	&  &\rulelabel{bwCon}
%	\\[.1cm]
%	\quad $\bwred\ \   \ptag{t_1}\requestAct{a}{x}{P_1}\ \mid \ \ptag{t_2}\acceptAct{a}{y}{P_2}$
%	%	
%	\\[.5cm]		
%	%
%	$\ptag{t_1}\sendAct{\ce{k}}{e}{P_1} \ \mid \ \ptag{t_2}\receiveAct{k}{x}{P_2}$
%	& $(k=s\ \, \text{or}\ \, k=\ce{s})$ &\rulelabel{fwCom}
%	\\[.1cm]
%	\quad $\fwred\ \  \res{t_1',t_2'}(
%	\ptag{t_1'}P_1 \mid \ptag{t_2'}P_2\subst{v}{x}
%	\mid \amem{\actEv{t_1}{\comAct{k}{e}{x}{P_1}{P_2}}{t_2}}{t_1'}{t_2'})$
%	&  $\expreval{e}{v}$ &
%	\\[.3cm]
%	$\res{t_1',t_2'}(\ptag{t_1'}P \mid \ptag{t_2'}Q
%	\mid \amem{\actEv{t_1}{\comAct{k}{e}{x}{P_1}{P_2}}{t_2}}{t_1'}{t_2'}$)
%	&  &\rulelabel{bwCom}
%	\\[.1cm]
%	\quad $\bwred\ \   \ptag{t_1}\sendAct{\ce{k}}{e}{P_1} \ \mid \ \ptag{t_2}\receiveAct{k}{x}{P_2}$
%	%	
%	\\[.5cm]		
%	%
%        $\ptag{t_1}\selectAct{\ce{k}}{l_i}{P} \ \mid \ 
%        \ptag{t_2}\branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}$
%	& $(k=s\ \, \text{or}\ \, k=\ce{s})$ &\rulelabel{fwLab}
%	\\[.1cm]
%	\quad $\fwred\ \  \res{t_1',t_2'}(
%	\ptag{t_1'}P \mid \ptag{t_2'}P_i
%	\mid \amem{\actEv{t_1}{\selAct{k}{l_i}{P}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}}{t_2}}{t_1'}{t_2'})$
%	&  $1 \leq i \leq n$ &
%	\\[.3cm]
%	$\res{t_1',t_2'}(\ptag{t_1'}Q \mid \ptag{t_2'}Q'
%	\mid \amem{\actEv{t_1}{\selAct{k}{l_i}{P}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}}{t_2}}{t_1'}{t_2'})$
%	&  &\rulelabel{bwLab}
%	\\[.1cm]
%	\quad $\bwred\ \   \ptag{t_1}\selectAct{\ce{k}}{l_i}{P} \ \mid \ 
%        \ptag{t_2}\branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}$
%	%	
%	\\[.5cm]		
%	%
%        $\ptag{t}\ifthenelseAct{e}{P_1}{P_2} 
%        \ \ \fwred\ \  \res{t'}(\ptag{t'}P_1
%	\mid \cmem{t}{\ifEv{e}{P_1}{P_2}}{t'})$
%	& $\expreval{e}{\ctrue}$ &\rulelabel{fwIf1}
%	\\[.3cm]
%        $\ptag{t}\ifthenelseAct{e}{P_1}{P_2} 
%        \ \ \fwred\ \  \res{t'}(\ptag{t'}P_2
%	\mid \cmem{t}{\ifEv{e}{P_1}{P_2}}{t'})$
%	& $\expreval{e}{\cfalse}$ &\rulelabel{fwIf2}	
%	\\[.3cm]		
%	$\res{t'}(\ptag{t'}P \mid \cmem{t}{\ifEv{e}{P_1}{P_2}}{t'})
%	\ \ \bwred\ \
%	\ptag{t}\ifthenelseAct{e}{P_1}{P_2}$
%	&  &\rulelabel{bwIf}
%	%	
%	\\[.5cm]		
%	%
%	\end{tabular}
%	\begin{tabular}{@{}c@{}}
%	$
%	\infer[$\ \rulelabel{fwPar}$]{M \mid \ N \ \fwred\ M' \mid N}
%	{M \ \fwred\ M'}
%	$	
%	\qquad\
%	$
%	\infer[$\ \rulelabel{fwRes}$]{\res{h}M \ \fwred\ \res{h}M'}
%	{M \ \fwred\ M'}
%	$
%	\qquad\
%	$
%	\infer[$\ \rulelabel{fwStr}$]{M \ \fwred\ N}
%	{M \congr M'\ \fwred\ N' \congr N}
%	$
%	%
%	\\[.5cm]
%	%
%	$
%	\infer[$\ \rulelabel{bwPar}$]{M \mid \ N \ \bwred\ M' \mid N}
%	{M \ \bwred\ M'}
%	$	
%	\qquad\
%	$
%	\infer[$\ \rulelabel{bwRes}$]{\res{h}M \ \bwred\ \res{h}M'}
%	{M \ \bwred\ M'}
%	$
%	\qquad\
%	$
%	\infer[$\ \rulelabel{bwStr}$]{M \ \bwred\ N}
%	{M \congr M'\ \bwred\ N' \congr N}
%	$
%	\\[.2cm]
%	\hline	
%	\end{tabular}
%	\vspace*{-.2cm}
%	\caption{\respi\ reduction relation}
%	\label{fig:reduction_respi}
%	%\vspace*{-.4cm}
%	\end{centering}
%\end{figure}
\begin{figure}[!t]
	\begin{centering}
	\begin{tabular}{@{}l@{\hspace*{-.6cm}}r@{\quad}l@{}}
	$\ptag{t_1}\requestAct{a}{x}{P_1}\ \mid \ \ptag{t_2}\acceptAct{a}{y}{P_2}$
	& $s,\ce{s} \notin \freese{P_1,P_2}$ &\rulelabel{fwCon}
	\\[.1cm]
	\quad $\fwred\ \  \res{s,t_1',t_2'}(
	\ptag{t_1'}P_1\subst{\ce{s}}{x} \mid \ptag{t_2'}P_2\subst{s}{y}$
	\\ \hspace{2.4cm}
	$\mid \amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'})$
	\\[.3cm]
	$\res{s,t_1',t_2'}(\ptag{t_1'}P \mid \ptag{t_2'}Q 
	\mid \amem{\actEv{t_1}{\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'})$
	&  &\rulelabel{bwCon}
	\\[.1cm]
	\quad $\bwred\ \   \ptag{t_1}\requestAct{a}{x}{P_1}\ \mid \ \ptag{t_2}\acceptAct{a}{y}{P_2}$
	%	
	\\[.5cm]		
	%
	$\ptag{t_1}\sendAct{\ce{k}}{e}{P_1} \ \mid \ \ptag{t_2}\receiveAct{k}{x}{P_2}$
	& $(k=s\ \, \text{or}\ \, k=\ce{s})$ &\rulelabel{fwCom}
	\\[.1cm]
	\quad $\fwred\ \  \res{t_1',t_2'}(
	\ptag{t_1'}P_1 \mid \ptag{t_2'}P_2\subst{v}{x}$
	&  $\expreval{e}{v}$ &
	\\
	\hspace*{2.1cm}
	$\mid \amem{\actEv{t_1}{\comAct{k}{e}{x}{P_1}{P_2}}{t_2}}{t_1'}{t_2'})$	
	\\[.3cm]
	$\res{t_1',t_2'}(\ptag{t_1'}P \mid \ptag{t_2'}Q
	\mid \amem{\actEv{t_1}{\comAct{k}{e}{x}{P_1}{P_2}}{t_2}}{t_1'}{t_2'}$)
	&  &\rulelabel{bwCom}
	\\[.1cm]
	\quad $\bwred\ \   \ptag{t_1}\sendAct{\ce{k}}{e}{P_1} \ \mid \ \ptag{t_2}\receiveAct{k}{x}{P_2}$
	%	
	\\[.5cm]		
	%
        $\ptag{t_1}\selectAct{\ce{k}}{l_i}{P} \ \mid \ 
        \ptag{t_2}\branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}$
	& $(k=s\ \, \text{or}\ \, k=\ce{s})$ &\rulelabel{fwLab}
	\\[.1cm]
	\quad $\fwred\ \  \res{t_1',t_2'}(
	\ptag{t_1'}P \mid \ptag{t_2'}P_i$
	&  $1 \leq i \leq n$ &
	\\
	\hspace*{2.1cm}
	$\mid \amem{\actEv{t_1}{\selAct{k}{l_i}{P}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}}{t_2}}{t_1'}{t_2'})$	
	\\[.3cm]
	$\res{t_1',t_2'}(\ptag{t_1'}Q \mid \ptag{t_2'}Q'$\\
	\hspace*{1.1cm}
	$\mid \amem{\actEv{t_1}{\selAct{k}{l_i}{P}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}}{t_2}}{t_1'}{t_2'})$
	&  &\rulelabel{bwLab}
	\\[.1cm]
	\quad $\bwred\ \   \ptag{t_1}\selectAct{\ce{k}}{l_i}{P} \ \mid \ 
        \ptag{t_2}\branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}$
	%	
	\\[.5cm]		
	%
        $\ptag{t}\ifthenelseAct{e}{P_1}{P_2} 
        \ \ \fwred\ \  \res{t'}(\ptag{t'}P_1
	\mid \cmem{t}{\ifEv{e}{P_1}{P_2}}{t'})$
	& $\expreval{e}{\ctrue}$ &\rulelabel{fwIf1}
	\\[.3cm]
        $\ptag{t}\ifthenelseAct{e}{P_1}{P_2} 
        \ \ \fwred\ \  \res{t'}(\ptag{t'}P_2
	\mid \cmem{t}{\ifEv{e}{P_1}{P_2}}{t'})$
	& $\expreval{e}{\cfalse}$ &\rulelabel{fwIf2}	
	\\[.3cm]		
	$\res{t'}(\ptag{t'}P \mid \cmem{t}{\ifEv{e}{P_1}{P_2}}{t'})
	\ \ \bwred\ \
	\ptag{t}\ifthenelseAct{e}{P_1}{P_2}$
	&  &\rulelabel{bwIf}
	%	
	\\[.5cm]		
	%
	\end{tabular}
	\begin{tabular}{@{\hspace{.9cm}}c@{\hspace{.9cm}}}
	$
	\infer[$\ \rulelabel{fwPar}$]{M \mid \ N \ \fwred\ M' \mid N}
	{M \ \fwred\ M'}
	$	
	\qquad\qquad
	$
	\infer[$\ \rulelabel{bwPar}$]{M \mid \ N \ \bwred\ M' \mid N}
	{M \ \bwred\ M'}
	$
	%
	\\[.5cm]
	%
	$
	\infer[$\ \rulelabel{fwRes}$]{\res{h}M \ \fwred\ \res{h}M'}
	{M \ \fwred\ M'}
	$
	\qquad\qquad
	$
	\infer[$\ \rulelabel{bwRes}$]{\res{h}M \ \bwred\ \res{h}M'}
	{M \ \bwred\ M'}
	$
	%
	\\[.5cm]
	%
	$
	\infer[$\ \rulelabel{fwStr}$]{M \ \fwred\ N}
	{M \congr M'\ \fwred\ N' \congr N}
	$	
	\qquad\qquad
	$
	\infer[$\ \rulelabel{bwStr}$]{M \ \bwred\ N}
	{M \congr M'\ \bwred\ N' \congr N}
	$
	\\[.2cm]
	\hline	
	\end{tabular}
	\vspace*{-.4cm}
	\caption{\respi\ reduction relation}
	\label{fig:reduction_respi}
	\vspace*{-.6cm}
	\end{centering}
\end{figure}

We comment on salient points. 
%
When two parallel threads synchronise to establish a new session (rule \rulelabel{fwCon}),
two fresh tags are created to uniquely identify the two continuations
of the synchronising threads. Moreover, all relevant information is stored in 
the action memory $\amem{\actEv{t_1}{\,\initAct{a}{x}{y}{P_1}{P_2}{s}}{t_2}}{t_1'}{t_2'}$: 
the tag $t_1$ of the initiator (i.e., the thread executing a prefix of the form
$\bar{a}(\cdot)$), the tag $t_2$ of the thread executing the dual action, 
the tags $t_1'$ and $t_2'$ of their continuations, 
the shared channel $a$ used for the synchronisation, the replaced variables $x$ and $y$,
the generated session channel $s$, 
and the processes $P_1$ and $P_2$ to which substitutions are applied. 
All such information is exploited to revert this reduction (rule \rulelabel{bwCon}).
In particular, the corresponding backward reduction is triggered by the
coexistence of the memory described above with two threads tagged 
$t_1'$ and $t_2'$, all of them within the scope of the session channel $s$
and tags $t_1'$ and $t_2'$ generated by the forward reduction (which, in fact, are 
removed by the backward one).
%
Notice that, when considering reachable processes,
due to tag uniqueness, the two processes $P$ and $Q$
must coincide with $P_1\subst{\ce{s}}{x}$ and $P_2\subst{s}{y}$;
indeed, as registered in the memory, these latter processes have 
been tagged with $t_1'$ and $t_2'$ by the forward reduction. 
Therefore, the fact that two threads tagged with $t_1'$ and $t_2'$ are 
available in parallel to the memory ensures that all actions possibly executed by 
the two continuations activated by the forward computation have been undone and, 
hence, we can safely proceed to undone the forward computation itself. 

Rules \rulelabel{fwCom}, \rulelabel{bwCom}, \rulelabel{fwLab}, \rulelabel{bwLab},
\rulelabel{fwIf1}, \rulelabel{fwIf2} and \rulelabel{bwIf} are similar. 
Notably, in the first two rules mentioned above, besides tags and continuation processes, 
the action memory stores the session endpoint $k$ of the 
receiving party (the other endpoint $\ce{k}$ is obtained by duality), the expression $e$ 
generating the sent value, and the replaced variable $x$. 
It is also worth noticing that, since all information about a choice event is stored in the 
corresponding memory, we need just one backward rule (\rulelabel{bwIf}) to revert the effect
of the forward rules \rulelabel{fwIf1} and \rulelabel{fwIf2}.
Finally, the meaning of the remaining rules, dealing with parallel composition, restriction  
and structural congruent terms, is straightforward. 


\begin{remark}[On memory information]
According to the rules in Figure~\ref{fig:reduction_respi}, when a forward reduction takes place
all information characterising the term generating the reduction is stored in a memory. 
Anyway, for what concerns the corresponding backward reduction, not all such information 
is always necessary. For example, in rule \emph{\rulelabel{fwCom}}, we could avoid memorizing 
process $P_1$, i.e.~the continuation of the sending thread, because it is not subject 
to substitution and, hence, it could be directly retrieved from the thread $t_1'$ in parallel with the memory. 
Thus, the backward rule \emph{\rulelabel{bwCom}} could be defined as follows:
$$  
\begin{array}{l}
\res{t_1',t_2'}(\ptag{t_1'}P_1 \mid \ptag{t_2'}Q
\mid \amem{\actEv{t_1}{\comAct{k}{e}{x}{}{P_2}}{t_2}}{t_1'}{t_2'})\\[.1cm]	
\ \ \bwred\ \   \ptag{t_1}\sendAct{\ce{k}}{e}{P_1} \ \mid \ \ptag{t_2}\receiveAct{k}{x}{P_2}
\end{array}
$$ 
Similarly, in rule \emph{\rulelabel{fwLab}}, no substitution is applied to 
the continuation processes, thus we could refrain from storing processes $P$ and $P_i$ in the memory.

However, in this work we are not interested in optimising the size of the data stored in the 
memories. Moreover, storing all information about forward reductions permits to determine the 
term producing the reduction without resorting to contextual information from terms in parallel with 
the considered memory. This shall be convenient when type checking memories. 
\end{remark}


\subsection{Multiple providers scenario: \respi}\label{sec:examplerespi}
Let us come back to the scenario introduced in Section~\ref{sec:intro} and 
specified in \pic\ in Section~\ref{sec:example}. 
We can obtain a \respi\ specification of the scenario by simply annotating 
the \pic\ term with (unique) tags as follows:
$$
\ptag{t_1}P_{client}  \ \mid \ \ptag{t_2}P_{provider1}  \ \mid \ \ptag{t_3}P_{provider2}  
$$

The computation described in Section~\ref{sec:example} corresponds to the 
following sequence of forward reductions:
$$
\begin{array}{l@{\ }l}
\multicolumn{2}{l}{
\ptag{t_1}P_{client}  \ \mid \ \ptag{t_2}P_{provider1}  \ \mid \ \ptag{t_3}P_{provider2}  
}
\\[.1cm]
\multicolumn{2}{l}{
\fwred\ \fwred\ \fwred\ \fwred\ \fwred
}
\\[.1cm]
M \ = & \res{s,t_1^1,t_2^1,t_1^2,t_2^2,t_1^3,t_2^3,t_1^4,t_1^5,t_2^4}
\\[.08cm]
&
(\,\ptag{t_1^5}P_{acc}\subst{\ce{s}}{x}\subst{\mathsf{quote}}{y_{quote}} \ \mid \
\ptag{t_2^4}Q_{acc}\subst{s}{y}\subst{\mathsf{srv\_req}}{z_{req}} 
\\[.08cm]
&
\ \ \mid \
\amem{\actEv{t_1}{\initAct{a_{login}}{x}{y}{P_{client}'}{P_{provider1}'}{s}}{t_2}}{t_1^1}{t_2^1}
\\[.08cm]
&
\ \ \mid \
\amem{\actEv{t_1^1}{\comAct{s}{\mathsf{srv\_req}}{z_{req}}{P_{client}''}{P_{provider1}''}}{t_2^1}}{t_1^2}{t_2^2}
\\[.08cm]
&
\ \ \mid \
\amem{\actEv{t_2^2}{\comAct{\ce{s}}{\mathsf{quote}}{y_{quote}}{P_{provider1}'''}{P_{client}'''}}{t_1^2}}{t_2^3}{t_1^3}
\\[.08cm]
&
\ \ \mid \
\cmem{t_1^3}{\ifEv{accept(\mathsf{quote})}{P_{client\_t}}{P_{client\_e}}}{t_1^4}
\\[.08cm]
&
\ \ \mid \
\amem{\actEv{t_1^4}{\selAct{s}{l_{acc}}{P_{acc}\subst{\ce{s}}{x}\subst{\mathsf{quote}}{y_{quote}}\\ 
&\hspace*{1.45cm} 
}{\branch{l_{acc}}{Q_{acc}\subst{s}{y}\subst{\mathsf{srv\_req}}{z_{req}}} \branchSep \ldots }}{t_2^3}}{t_1^5}{t_2^4}
\,)
\\
&
\mid \ P_{provider2}  
\end{array}
$$

Now, if a problem occurs during the subsequent interactions between the client and the provider for 
finalising the service agreement, the computation can be reverted to initial state, in order to allow 
the client to start a new session with (possibly) another provider. 
$$
M \ \bwred\ \bwred\ \bwred\ \bwred\ \bwred\ \ptag{t_1}P_{client}  \ \mid \ \ptag{t_2}P_{provider1}  \ \mid \ \ptag{t_3}P_{provider2}  
$$
Notice that in the reversible calculus there is no need of explicitly implementing loops 
for enabling the client to undo and restart sessions. Notice also that here we do not consider 
specific primitives and techniques for avoiding interacting again with the same provider.
They should break the Loop Lemma (see Lemma~\ref{lemma:loop}) and complicate 
our theoretical framework; we refer to \cite{LaneseMS12} for a definition of 
some of such controlled forms of reversibility.







==> tex/types.tex <==
% !TEX root = ../reversible_sessions_TR.tex
\section{Type discipline}
\label{sec:types}

In this section, first we define the session type discipline of the session-based \pic\
introduced in Section~\ref{sec:host_calculus}, then we discuss how we could extend it 
in order to type \respi\ processes introduced in Section~\ref{sec:rev_calculus}.

\subsection{Typing session-based \pic}
\label{sec:typingPic}

The type discipline presented here is a minor revision of the one proposed in 
\cite{YoshidaV07}, that takes into account the changes applied to the considered 
variant of \pic\ (discussed in Section~\ref{sec:syntax_pic}).

\subsubsection{Types}
The syntax of \emph{sorts}, ranged over by $S$, $S'$, \ldots, and \emph{types}, ranged over by $\alpha$, 
$\beta$, \ldots, is defined in Figure~\ref{fig:typeSyntax}.
%
\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{rcl@{\hspace{-.1cm}}r}
	\textbf{Sorts}\quad
	$S$ & ::= & $\boolType$ & boolean\\
	& $\mid$ & $\intType$ & integer\\
	& $\mid$ & $\sharedChanType{\alpha}$ & shared channel\\
	\\
	\textbf{Types}\quad
	$\alpha$ & ::= & $\outType{S}.\alpha$ & output\\	
	& $\mid$ & $\inpType{S}.\alpha$ & input\\		
	& $\mid$ & $\thrType{\beta}.\alpha$ & throw\\		
	& $\mid$ & $\catType{\beta}.\alpha$ & catch\\			
	& $\mid$ & $\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ & selection\\			
	& $\mid$ & $\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ & branching\\				
	& $\mid$ & $\inactType$ & end
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Syntax of sorts and types}
	\label{fig:typeSyntax}
	\vspace*{-.4cm}
	\end{centering}
\end{figure}
%
The type $\outType{S}.\alpha$ represents the behaviour of first outputting a value of sorts $S$, 
then performing the actions prescribed by type $\alpha$; 
type $\thrType{\beta}.\alpha$ represents a similar behaviour, which starts with session output 
(\emph{throw}) instead; 
types $\inpType{S}.\alpha$ and $\catType{\beta}.\alpha$ are the dual ones, 
receiving values instead of sending. 
%
Type $\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ describes a branching 
behaviour: it waits with $n$ options, and behave as type $\alpha_i$ if the $i$-th action is selected 
(external choice); 
type $\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ then represents the behaviour 
which would select one of $l_i$ and then behaves as $\alpha_i$, according to the selected $l_i$ 
(internal choice). Type $\inactType$ represents inaction, acting as the unit of sequential composition.

For each type $\alpha$, we define $\dual{\alpha}$, the \emph{dual type} of $\alpha$, 
by exchanging $!$ and $?$, and $\&$ and $\oplus$. The inductive definition is in Figure~\ref{fig:dualType}.
%
\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{r@{\ }c@{\ }l@{\qquad}r@{\ }c@{\ }l@{\qquad}r@{\ }c@{\ }l@{\qquad}r@{\ }c@{\ }l}
	$\dual{\outType{S}.\alpha}$ & = & $\inpType{S}.\dual{\alpha}$
	&
	$\dual{\outType{\beta}.\alpha}$ & = & $\inpType{\beta}.\dual{\alpha}$	
	&
	$\dual{\selType{\branch{l_i}{\alpha_i}}_{i\in I}}$ & = & $\branchType{\branch{l_i}{\dual{\alpha_i}}}_{i\in I}$
	&
	$\dual{\inactType}$ & = & $\inactType$
	\\[.3cm]
	$\dual{\inpType{S}.\alpha}$ & = & $\outType{S}.\dual{\alpha}$	
	&
	$\dual{\inpType{\beta}.\alpha}$ & = & $\outType{\beta}.\dual{\alpha}$	
	&
	$\dual{\branchType{\branch{l_i}{\alpha_i}}_{i\in I}}$ & = & $\selType{\branch{l_i}{\dual{\alpha_i}}}_{i\in I}$	
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Dual types}
	\label{fig:dualType}
	%\vspace*{.4cm}
	\end{centering}
\end{figure}
%

\subsubsection{Typing System}
A \emph{sorting} (resp. a \emph{typing}, resp. a \emph{basis}) is a finite partial map from 
shared identifiers to sorts (resp. from session identifiers to types, resp. from process variables to typings). 
We let $\sorting$, $\sorting'$, \ldots (resp. $\typing$, $\typing'$, \ldots, 
resp. $\basis$, $\basis'$, \ldots) range over sortings (resp. typings, resp. bases).
%
We write $\typing \comp k:\alpha$ when $k \notin dom(\typing)$;
this notation is then extended to $\typing \comp \typing'$. 

Typing judgement are of the form $\basis;\sorting \judge P \hasType \typing$
which stands for ``under the environment $\basis;\sorting$, process $P$ has typing $\typing$''. 
The typing system is defined by the axioms and rules in Figure~\ref{fig:typingSysytem}. 
We call a typing \emph{completed} when it contains only $\inactType$ types. 
A typing $\typing$ is called \emph{balanced} if  whenever $s:\alpha,\ce{s}:\beta\in \typing$, then $\alpha=\dual{\beta}$.
%
We refer the interested reader to \cite{YoshidaV07} for detailed comments on the rules
and results.

\begin{figure}[!t]
	\begin{centering}
	\begin{tabular}{@{\hspace*{-2cm}}c}
	$\sorting \judge \ctrue \hasType \boolType$\ \ \rulelabel{Bool$_{\mathit{tt}}$}
	\qquad
	$\sorting \judge \cfalse \hasType \boolType$\ \ \rulelabel{Bool$_{\mathit{ff}}$}
	\qquad
	$\sorting \judge 1 \hasType \intType$\ \ \rulelabel{Int}	
	\qquad \ldots
	\\[.4cm]
	$
	\infer[$\ \rulelabel{Sum}$]{\sorting \judge +(e_1,e_2) \hasType \intType}
	{\sorting \judge e_1 \hasType \intType & & \sorting \judge e_2 \hasType \intType}
	$		
	\qquad
	$
	\infer[$\ \rulelabel{And}$]{\sorting \judge \wedge(e_1,e_2) \hasType \boolType}
	{\sorting \judge e_1 \hasType \boolType & & \sorting \judge e_2 \hasType \boolType}
	$		
	\qquad \ldots
	\\[.2cm]
	\end{tabular}
	\begin{tabular}{@{\hspace*{-2cm}}r@{\hspace*{.4cm}}r}
	$\sorting\comp u:S \judge u \hasType S$\ \ \rulelabel{Id}	
	&
	\infer[$\ \rulelabel{Inact}$]{\basis;\sorting \judge \inact \hasType \typing}
	{\typing\ \  \text{completed}}	
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Req}$]{\basis;\sorting \judge \requestAct{u}{x}{P} \hasType \typing}
	{\sorting \judge u \hasType \sharedChanType{\alpha} & & \basis;\sorting \judge P \hasType \typing\comp x:\dual{\alpha}}
	$		
	&
	$
	\infer[$\ \rulelabel{Acc}$]{\basis;\sorting \judge \acceptAct{u}{x}{P} \hasType \typing}
	{\sorting \judge u \hasType \sharedChanType{\alpha} & & \basis;\sorting \judge P \hasType \typing\comp x:\alpha}
	$		
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Send}$]{\basis;\sorting \judge \sendAct{k}{e}{P} \hasType \typing\comp k:\outType{S}.\alpha}
	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType \typing\comp k:\alpha}
	$		
	&
	$
	\infer[$\ \rulelabel{Thr}$]{\basis;\sorting \judge \sendAct{k}{k'}{P} \hasType \typing\comp k:\thrType{\alpha}.\beta\comp k':\alpha}
	{\basis;\sorting \judge P \hasType \typing\comp k:\beta}
	$		
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Rcv}$]{\basis;\sorting \judge \receiveAct{k}{x}{P} \hasType \typing\comp k:\inpType{S}.\alpha}
	{\basis;\sorting\comp x:S \judge P \hasType \typing\comp k:\alpha}
	$		
	&
	$
	\infer[$\ \rulelabel{cat}$]{\basis;\sorting \judge \receiveAct{k}{x}{P} \hasType \typing\comp k:\catType{\alpha}.\beta}
	{\basis;\sorting \judge P \hasType \typing\comp k:\beta \comp x:\alpha}
	$		
	\\[.4cm]	
	\multicolumn{2}{c}{	
	$
	\infer[(1 \leq j \leq n)\  $\ \rulelabel{Sel}$]{\basis;\sorting \judge \selectAct{k}{l_j}{P} \hasType \typing
	\comp k:\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}}
	{\basis;\sorting  \judge P \hasType \typing \comp k:\alpha_j}
	$}
	\\[.4cm]	
	\multicolumn{2}{c}{	
	$
	\infer[$\ \rulelabel{Br}$]{\basis;\sorting \judge \branchAct{k}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}} \hasType \typing
	\comp k:\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}}
	{\basis;\sorting  \judge P_1 \hasType \typing \comp k:\alpha_1 && \ldots 
	 && \basis;\sorting  \judge P_n \hasType \typing \comp k:\alpha_n}
	$}
	\\[.4cm]		
	\multicolumn{2}{c}{
	$
	\infer[$\ \rulelabel{If}$]{\basis;\sorting \judge \ifthenelseAct{e}{P}{Q} \hasType \typing}
	{\sorting  \judge e \hasType \boolType &&
	\basis;\sorting  \judge P \hasType \typing && \basis;\sorting  \judge Q \hasType \typing}
	$}	
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Conc}$]{\basis;\sorting \judge P\mid Q \hasType \typing\comp \typing'}
	{\basis;\sorting  \judge P \hasType \typing && \basis;\sorting  \judge Q \hasType \typing'}
	$		
	&
	$
	\infer[$\ \rulelabel{Res1}$]{\basis;\sorting \judge \res{a}{P} \hasType \typing}
	{\basis;\sorting\comp a:S  \judge P \hasType \typing}
	$	
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Res2}$]{\basis;\sorting \judge \res{s}{P} \hasType \typing}
	{\basis;\sorting  \judge P \hasType \typing\comp s:\alpha \comp \ce{s}:\dual{\alpha}}
	$	
	&
	$
	\infer[$\ \rulelabel{Res3}$]{\basis;\sorting \judge \res{s}{P} \hasType \typing}
	{\basis;\sorting  \judge P \hasType \typing && s\ \text{ not in }\ \typing}
	$	
	\\[.4cm]	
	$\basis\comp X:\typing;\sorting \judge X \hasType \typing$\ \ \rulelabel{Var}			
	&
	\infer[$\ \rulelabel{Rec}$]{\basis;\sorting \judge \recAct{X}{P} \hasType \typing}
	{\basis\comp X:\typing;\sorting  \judge P \hasType \typing}	
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}
	\caption{Typing System for \pic}
	\label{fig:typingSysytem}
	%\vspace*{-.4cm}
	\end{centering}
\end{figure}



\subsection{Towards typing \respi}\label{sec:typeSystemRespi}

%The first question that must be answered before
A question that should be answered before defining a type discipline for a reversible 
calculus is ``\emph{Should we type check the processes stored in the memories?}''.
%
The question arises from the fact that we should be able to determine if any \respi\ process is well-typed or not. 
%
Indeed, if the answer would be ``\emph{No}'', it would be sufficient to convert a 
process of the reversible calculus into the corresponding process of the host calculus, by applying 
the forgetful map $\forgetMap$ (Definition~\ref{def:forgetfulMap}), and then to type check 
the latter process by using the typing system defined for the host calculus
(Section~\ref{sec:typingPic}). 
%
However, in our case the answer to the question is ``\emph{Yes}'', because otherwise 
typability would not be preserved under reduction (i.e.,  Subject Reduction Theorem would not 
be satisfied).
We show this with a simple example. 

Let us consider the following \respi\ process (we omit trailing occurrences of~$\inact$):
$$
\begin{array}{l}
M \ = \ \res{s,t_1',t_2',t_2''}\\
\hspace{1.1cm}
(\,
\ptag{t_1'}\receive{\ce{s}}{x} \mid
\ptag{t_2''}\send{s}{1+1} \mid
\amem{\actEv{t_1}{\comAct{s}{1}{y}{P_1}{P_2}}{t_2}}{t_1'}{t_2'} 
\\
\hspace{1.3cm}
\mid
\cmem{t_2'}{\ifEv{(1>0)}{(\send{s}{1+1})}{(\send{s}{\cfalse})}}{t_2''}
\,)
\end{array}
$$
where 
$P_1 = \receive{\ce{s}}{x}$ and 
$P_2 = \ifthenelseAct{(y>0)}{\send{s}{y+1}}{\send{s}{\cfalse}}$.
Intuitively, in previous reductions the thread $t_1$ sent 
the value $1$ to the thread $t_2$;  then the received value has been 
used by the continuation of $t_2$, i.e. the thread $t_2'$, to evaluate
a conditional choice. 

The corresponding \pic\ process is 
$$
\begin{array}{l}
\forget{M} \ = \ \res{s}
(\,
\receive{\ce{s}}{x} \mid
\send{s}{1+1} 
\,)
\end{array}
$$
which can be typed as follows:
$$
\scriptsize
\infer[$\ \rulelabel{Res2}$]{\emptyset;\emptyset \judge 
\res{s}{(\receiveAct{\ce{s}}{x}{\inact} \mid \sendAct{s}{1+1}{\inact})}
\hasType \emptyset}
{
\infer[$\ \rulelabel{Conc}$]{\emptyset;\emptyset \judge 
\receiveAct{\ce{s}}{x}{\inact} \mid
\sendAct{s}{1+1}{\inact} \hasType  \ce{s}:\inpType{\intType}.\inactType \comp s:\outType{\intType}.\inactType}
{
\infer[$\ \rulelabel{Rcv}$]{\emptyset;\emptyset 
\judge \receiveAct{\ce{s}}{x}{\inact}  \hasType \ce{s}:\inpType{\intType}.\inactType}
{
\infer[$\ \rulelabel{Inact}$]{\emptyset;x:\intType \judge \inact \hasType \ce{s}:\inactType}{}
}
&& 
\infer[$\ \rulelabel{Send}$]{\emptyset;\emptyset \judge \sendAct{s}{1+1}{\inact} \hasType s:\outType{\intType}.\inactType}
{
	\infer[$\ \rulelabel{Sum}$]{\emptyset \judge 1+1 \hasType \intType}
	{\infer[$\ \rulelabel{Int}$]{\emptyset \judge 1 \hasType \intType}{} }
&& 
\infer[$\ \rulelabel{Inact}$]{\emptyset;\emptyset \judge \inact \hasType s:\inactType}{}}
}
}
$$

However, process $M$ can perform a backward reduction and evolve to:
$$
\begin{array}{@{}l@{}}
M' \, = \, \res{s,t_1',t_2'}
(\,
\ptag{t_1'}\receive{\ce{s}}{x} \mid
\ptag{t_2'}\ifthenelseAct{(1>0)}{\send{s}{1+1}}{\send{s}{\cfalse}}
\\\
\hspace*{2.7cm}
\mid
\amem{\actEv{t_1}{\comAct{s}{1}{y}{P_1}{P_2}}{t_2}}{t_1'}{t_2'} 
\,)
\end{array}
$$
Unfortunately, $\forget{M'}$ is not typable, because the then-branch of the conditional choice
is only typable under typing $s:\outType{\intType}.\inactType$ while 
the else-branch under typing $s:\outType{\boolType}.\inactType$ and, therefore,
the conditional choice is not typable (see rule \rulelabel{If} in Figure~\ref{fig:typingSysytem}).

%Now, since memories must be typed, one could wonder if it is possible to type 
%\respi\ processes in a na\"ive compositional way, i.e. by type checking terms different 
%from memories by resorting to the typing system in Figure~\ref{fig:typingSysytem}
%(thus, ignoring tags) and by type checking each memory by checking (again with the
%same type system) the term producing the corresponding reduction. 
%Unfortunately, in general this approach does not work. 
%Consider indeed the following \respi\ process:
Now, since memories must be typed, one could wonder if it is possible to na\"ively type 
\respi\ processes by separately type checking the term
resulting from the application of $\forgetMap$ and each single memory, 
by using the typing system in \cite{YoshidaV07}. In particular, for each memory 
we would check the stored term that generated the memory. 
Unfortunately, in general this approach does not work. 
Consider indeed the following \respi\ process:
$$
\begin{array}{@{}l@{}}
N_1 \, = \, \res{s,t_2',t_4'}
(\,
\ptag{t_1}\send{\ce{s}}{1} \mid
\ptag{t_2'}\inact \mid
\ptag{t_3}\receive{s}{x} \mid
\ptag{t_4'}\inact
\mid
\amem{\actEv{t_2}{\comAct{s}{2}{y}{\inact}{\inact}}{t_4}}{t_2'}{t_4'} 
\,)
\end{array}
$$
By ignoring memory and tags, the rest of the term is typable 
under typing $\emptyset$, because 
$\send{\ce{s}}{1} \mid \receive{s}{x}$ is typable under typing
$\typing \,=\, \ce{s}:\outType{\intType}.\inactType \comp s:\inpType{\intType}.\inactType$.
Similarly, the term that performed the reduction generating the memory,
i.e. $\send{\ce{s}}{2} \mid \receive{s}{y}$, is typable under the same typing $\typing$.
%
However, $N_1$ can perform the following backward reduction:
$$
N_1  \bwred \res{s}
(\,
\ptag{t_1}\send{\ce{s}}{1} \mid
\ptag{t_2}\send{\ce{s}}{2} \mid
\ptag{t_3}\receive{s}{x} \mid
\ptag{t_4}\receive{s}{y} 
\,) \ = \ N_2
$$
and $\forget{N_2}$ is not typable, because the typings of its parallel processes  
are not composable (e.g., both $\send{\ce{s}}{1} \mid \receive{s}{x}$
and $\send{\ce{s}}{2} \mid \receive{s}{y}$ have typing $\typing$,
but $\typing \comp \typing$ is not defined). 

From this we learn that, in general, a memory cannot be type checked in isolation
without taking into account its context. 
%
Such context can be considered by extending the typing system 
in \cite{YoshidaV07} with rules that permits typing memories and ignoring tag annotations 
and tag restrictions.  In this way, typings of memories 
and of threads are composed by means of the rule for parallel composition. 
Thus, e.g., the process $N_1$ above is not typable by such typing system. 
%
However, type checking memories is a tricky task due to the dependencies 
among them and with the threads outside memories. 
If such dependencies would be ignored, unwanted conflicts during type checking could 
arise. Thus, an appropriate type discipline requires to type check only the memories
that do not depend on other memories; for each of them, we have to type check  
the stored process without considering as context threads and memories that depend 
on the memory under consideration. 

In this work, we consider a simplified setting that permits avoiding to deal with 
such dependencies. 
%
Specifically, we consider the class of \respi\ processes that are \emph{reachable from empty simple sessions},
i.e., by extending Definition~\ref{def:reachable}, 
processes obtained by means of forward and backward reductions from 
processes with unique tags, no memory, no session initialised, no conditional choices and 
recursions at top-level, and no delegation. 
The characteristic of such processes is the following one: for each memory  
inside a process, there exists within the process an ancestor memory 
corresponding to the initialisation of the considered session. Thus, we
can only focus on this latter kind of memories, which significantly simplifies 
the theory. 

Therefore, we slightly extend the typing system for \pic\ by adding the rules in Figure~\ref{fig:typingSysytem_respi}
to those in Figure~\ref{fig:typingSysytem} (rules extending 
\rulelabel{Res1}, \rulelabel{Res2} and \rulelabel{Res3} to \respi\ processes
in a natural way have been omitted).
We comment on salient points.
%
Process $\nil$ (rule \rulelabel{Nil}) is dealt with in a different way wit respect to $\inact$,
because the former does not indicate the end of a thread but 
just an empty process (which cannot be nested in action prefixes). 
Therefore, $\nil$ is typable under any environment and typing.
Rule \rulelabel{Thrd} permits ignoring tags and, hence, resorting to the typing system of 
\pic\ for checking threads. Similarly, rule \rulelabel{Res'} permits ignoring 
tag restrictions. 
Rule \rulelabel{Conc'} simply extends \rulelabel{Conc} to \respi\ processes.
Rule \rulelabel{Mem1} permits ignoring all memories but for those derived from 
a session initialisation, which are checked by means of rule \rulelabel{Mem2}
by resorting to the typing system of \pic\ for checking the generating term.  
Notably, some sessions could be checked more than once (in case the corresponding initialisation 
actions are nested in other processes), anyway this does not cause any conflict. 
Notice also, that stored processes are closed, since they have given rise to a reduction. 
%
Results about such typing system and definition of a type discipline for a broader 
class of \respi\ process are currently under investigation. 

\begin{figure}[t]
	\begin{centering}
	\begin{tabular}{r@{\ }r}
	$\basis;\sorting \judge \nil \hasType \typing$\ \ \rulelabel{Nil}
	&
	$
	\infer[$\ \rulelabel{Conc'}$]{\basis;\sorting \judge M\mid N \hasType \typing\comp \typing'}
	{\basis;\sorting  \judge M \hasType \typing && \basis;\sorting  \judge N \hasType \typing'}
	$		
	\\[.4cm]	
	$
	\infer[$\ \rulelabel{Res'}$]{\basis;\sorting \judge \res{t}{M} \hasType \typing}
	{\basis;\sorting  \judge M \hasType \typing}
	$	
	&
	\infer[$\ \rulelabel{Mem1}$]{\basis;\sorting \judge m \hasType \typing}
	{m \neq \amem{\actEv{t_1}{\initAct{a}{x}{y}{P}{Q}{s}}{t_2}}{t_1'}{t_2'}}		
	\\[.4cm]		
	\infer[$\ \rulelabel{Thrd}$]{\basis;\sorting \judge (\ptag{t}P) \hasType \typing}
	{\basis;\sorting \judge P \hasType \typing}	
	&
	\infer[$\ \rulelabel{Mem2}$]{\basis;\sorting \judge \amem{\actEv{t_1}{\initAct{a}{x}{y}{P}{Q}{s}}{t_2}}{t_1'}{t_2'} \hasType \typing}
	{\basis;\sorting \judge (\ptag{t_1}\requestAct{a}{x}{P}\ \mid \ \ptag{t_2}\acceptAct{a}{y}{Q}) \hasType \typing}	
	\\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Typing System for \respi\ (additional rules)}
	\label{fig:typingSysytem_respi}
	%\vspace*{-.4cm}
	\end{centering}
\end{figure}


\subsection{Multiple providers scenario: typing system}
Coming back to the scenario introduced in Section~\ref{sec:example}
and specified in \respi\ in Section~\ref{sec:examplerespi}, 
we can easily verify that the process
$$
\ptag{t_1}P_{client}  \ \mid \ \ptag{t_2}P_{provider1}  \ \mid \ \ptag{t_3}P_{provider2}  
$$
is well-typed with respect to the typing system discussed in Section~\ref{sec:typeSystemRespi}
(assuming that the unspecified processes $P_{acc}$, $P_{neg}$, $Q_{acc}$ and $Q_{neg}$
are properly typable). 
In particular, the channel $a_{login}$ can be typed by the shared channel type
$$
\sharedChanType{\,\inpType{\mathsf{Request}}.\,\outType{\mathsf{Quote}}.\,
\branchType{\branch{l_{acc}}{\alpha_{acc}}\,,\,\branch{l_{neg}}{\alpha_{neg}}\,,\,\branch{l_{rej}}{\inactType}}\,}
$$
where we use sorts $\mathsf{Request}$ and $\mathsf{Quote}$ to type requests and quotes,
respectively.

Let us consider now a scenario where the client wills to concurrently submit two different 
requests to the same provider, which would be able to concurrently serve them. 
Consider in particular the following specification of the client (the provider one is the dual):
$$
\begin{array}{l}
\requestPrefix{a_{login}}{x}.\,(\,\send{x}{\mathsf{srv\_req\_1}}.\,P_{1} \ \mid \ \send{x}{\mathsf{srv\_req\_2}}.\,P_{2} \,)
\end{array}
$$
The new specification of the scenario is clearly not well-typed, due to the use of 
parallel threads within the same session. This permits avoiding mixing up messages related to different 
requests and wrongly delivering them. In order to properly concurrently submit separate requests,
the client must instantiate separate sessions with the provider, one for each request.

The session type discipline, indeed, forces concurrent interactions to follow structured patterns 
that guarantee the correctness of communication. 
%
For what concerns reversibility, linear use of session channels limits the 
effect of causal consistency, since concurrent interactions along the same session 
are prevented and, hence, the backtracking of a given session follows a single path. 
Anyway, interactions along different sessions are still concurrent and, therefore, 
causal-consistent rollback can be applied to revert them.



